Enumerative geometry of $K3$ surfaces

The aim of these notes is to explain various enumerative results about $K3$ surfaces without assuming familiarity with Gromov--Witten theory. The enumerative results in question are due to Beauville, Bryan and Leung, Pandharipande, Maulik, Thomas, and others, and confirm conjectures made by Yau--Zaslow, G\"ottsche, and Katz--Klemm--Vafa.

==> K3enum.tex <==
\chaptitle{Enumerative geometry of $K3$ surfaces}
\chapauthor{Thomas Dedieu}

\startchap
\label{10.th-panoramico}



\newcommand{\ff}{\mathfrak{f}}

\newcommand{\ste}{\mathsf{e}}
\newcommand{\stf}{\mathsf{f}}
\newcommand{\sts}{\mathsf{s}}
\newcommand{\stT}{\mathsf{T}}

\newcommand{\cE}{\mathcal{E}}
\providecommand{\cK}{\mathcal{K}}
%\newcommand{\cC}{\mathcal{C}}

\newcommand{\Mp}{\mathrm{Mp}}
\newcommand{\bLK}{\mathbf{L}_{K3}}
\newcommand{\cJac}{\bar{\mathcal{J}}}
\newcommand{\Mbar}{\overline{M}}
\newcommand{\vdim}{\operatorname{vdim}}
\newcommand{\NL}{\mathrm{NL}}
\newcommand{\EG}{\mathrm{EG}}
\newcommand{\pt}{\mathrm{pt}}
\newcommand{\End}{\operatorname{End}}


% \newenvironment{perso}{\color{purple}}{}
% \newenvironment{taf}{\color{blue}}{}




\startcontents[panoramico]
\renewcommand{\tocdataformat}[1]{\null}
\printcontents[panoramico]{}{1}[2]{}


\section{Introduction}

The aim of these notes is to explain various enumerative results
about $K3$ surfaces without assuming familiarity with
Gromov--Witten theory; in fact, they represent an attempt on my part
to understand the meaning of these results in classical terms. 
The enumerative results in question are due to Beauville, Bryan and
Leung, Pandharipande, Maulik, Thomas, and others, and confirm
conjectures made by Yau--Zaslow, Göttsche, and Katz--Klemm--Vafa.
They are listed in Paragraph \ref{p:topics} below.

They fall in three categories:
(i) results that don't really need Gromov--Witten theory at all,
either to be formulated or to be proved;
(ii) results that may be formulated without Gromov--Witten theory,
but which necessitate techniques from this theory to be proven (as far
as current knowledge goes);
(iii) results which require an understanding of Gromov--Witten
theory to be fully appreciated.
The text provides the necessary background in Gromov--Witten theory in
order to understand results from all these three categories.
In particular we shall give a brief idea 
of what Gromov--Witten invariants are in Paragraph \ref{p:GW}.

\paragraph{Contents description}
\label{p:topics}
% Specifically, we shall discuss the following topics. 
In Section~\ref{S:YZ} we state a formula of Yau and Zaslow giving the
number of rational 
curves in a primitive linear system $|L|$ on a $K3$ surface $S$,
and give its
proof by Beauville following the strategy suggested by Yau--Zaslow,
using the universal compactified Jacobian; this falls in
the above mentioned category (i).
In this formula, each rational curve is counted with multiplicity
equal to the topological Euler number of its compactified Jacobian,
which depends only on the singularities of the curve.
We also present results due to
Fantechi, Göttsche, and van Straten
which show that this is also the multiplicity of the origin in a
semi-universal deformation space of the singularities of the curve.


The Yau--Zaslow formula is generalized in Section~\ref{S:GWK3} to a
formula giving the number of genus $g$ curves in the system $|L|$
passing through $g$ general points on $S$,
for arbitrary $g$; this generalized formula
had been conjectured by Göttsche.
We give an outline of its proof by Bryan and Leung,
by degeneration to an elliptic $K3$ surface, with as much details as the
scope of these notes and the ability of the author permit.
This proof requires
the formulation of the result in terms of some special version of
Gromov--Witten invariants specifically designed for algebraic $K3$
surfaces (see Section~\ref{s:red-th}), and relies among other things on a
multiple cover formula for nodal rational curves. This result thus
falls in category (ii).

Essentially all remaining results fall in category (iii).
The goal of Section~\ref{S:BPS} is to explain the extension of the
Yau--Zaslow formula to a formula for non-primitive linear systems,
which has been 
proven by Klemm--Maulik--Pandharipande--Scheidegger (this proof is
streamlined in Section~\ref{s:KMPSpf}). This features the
Aspinwall--Morrison multiple cover formula, and its application to
define corrected Gromov--Witten invariants known as BPS states
numbers. I also discuss other degenerate contributions to these
invariants besides plain multiple curves, striving to sort out the
relation between the number given by the formula and the actual number
of integral rational curves.

In Section~\ref{S:3fold} we introduce
various generalizations of the Gromov--Witten invariants on $K3$
surfaces considered so far, in particular the Hodge integrals and
their BPS states version.
The main theme in this section is the relation between 
between Gromov--Witten integrals on $K3$ surfaces and curve counting
Gromov--Witten invariants on threefolds. For
instance, we discuss the Katz--Klemm--Vafa formula, proved by
Pandharipande and Thomas, which may be seen as computing
the excess contribution of an algebraic $K3$ surface to the Gromov--Witten
invariants of any fibered threefold in which it appears as a fibre.
Some of the material presented in this section is necessary for the
proof (discussed in Section \ref{S:KMPS}) of the Yau--Zaslow formula for non
primitive classes (stated in Section \ref{S:BPS}).

In
Section~\ref{S:KMPS} we introduce Noether--Lefschetz numbers for
families of lattice-polarized $K3$ surfaces, and state a theorem due
to Maulik and Pandharipande which shows, 
on a threefold fibered in lattice-polarized $K3$ surfaces,
how these Noether--Lefschetz numbers give an explicit relation between
Gromov--Witten invariants of the threefold and of the $K3$ fibres.
Finally, we discuss the application of this formula to the proof of
the Yau--Zaslow formula for non-primitive linear systems.
It involves a mirror symmetry theorem that enables the computation of
Gromov--Witten invariants of anticanonical sections of toric
$4$-manifolds, 
as well as modularity results for Noether--Lefschetz numbers
following from the work of Borcherds and Kudla--Millson; the latter
enable the computation of all Noether--Lefschetz numbers of the family of
lattice-polarized $K3$ surfaces considered in the proof, viz.\ the
so-called $STU$ model.


\paragraph{Gromov--Witten theory}
\label{p:GW}
Let $X$ be a compact complex manifold.
In Gromov--Witten theory, one views genus $g$ curves
on $X$ as 
\emph{stable maps}, \ie morphisms $f: C \to X$ where $C$ is a
connected, nodal, 
curve of arithmetic genus $g$, such that there are only finitely many
automorphisms $\phi$ of $C$ satisfying the identity $f \circ \phi =f$.
The latter condition is called the \emph{stability condition}, and
amounts to the requirement that each irreducible component of
arithmetic genus $0$ (resp., $1$) of $C$ which is contracted by $f$
carries at least $3$ (resp., $1$)
\emph{special points}, \ie either
intersection points with other irreducible components of $C$ or, if
relevant, marked points.
An integral embedded curve $C \subset X$ is then encoded as the map
$f: \bar C \to X$ obtained by composing the normalization of $C$ with
its embedding in $X$.

Stable maps have moduli spaces that are compact.
Let $g$ and $k$ be non-negative integers, and $\beta$ be
a homology class in $H_2(X,\Z)$.
We denote by $\Mbar _{g,k} (X,\beta)$ the moduli space of genus $g$
stable maps $f: C \to X$, with $k$ marked points on $C$,
such that $[f_*(C)] =\beta$. It is compact, has expected dimension
\begin{equation}
\label{eq:vdim0}
\expdim \bigl(\, \Mbar_{g,k} (X, \beta) \bigr)
%&= \chi (N_f) + k \\
= (\dim (X) -3)(1-g) -K_X \cdot \beta + k,
\footnote
{at a point of $\Mbar_{g,k} (X, \beta)$ corresponding to a map
$f:C \to X$ such that $C$ is smooth and $f$ is unramified,
this may be computed as $\chi (N_f) + k$, where $N_f$ 
(the \emph{normal sheaf} of $f$) is the locally free cokernel of the
injective map of locally free sheaves $T_C \to f^* T_X$,
see \cite[Section \tref{S:deform-maps}]{02.edoardo},
\cite[\S~3.4.2]{edoardo}, or \cite[\S~1$\frac 1 2$]{pt-13/2};
these references also explain how to compute the expected dimension in
general.}
\end{equation}
and all its irreducible components have dimension larger than or equal
to the expected dimension.
The moduli space $\Mbar _{g,k} (X,\beta)$ has in general many
irreducible components, including some parametrizing stable maps that
one would arguably rather discard if one is willing to 
enumerate genuine curves on $X$: for instance, note that the
contraction of a curve $C$ of genus $g\geq 2$ to a point of $X$ is a
stable map.
It turns out nevertheless that considering stable maps instead of
embedded curves
provides much better behaved (\eg deformation invariant)
enumerative numbers.
It is possible to consider different devices instead of stable maps in
order to
obtain well-behaved enumerative numbers, each such possibility coming with
its own specific pros and cons; about this, 
see the enlightening survey \cite{pt-13/2}.


Now, Gromov--Witten invariants are\footnote
{in fact there are other Gromov--Witten invariants, which are
more general intersection numbers against
$[\Mbar_{g,k} (X, \beta)] ^{\rm vir}$
than those in \eqref{eq:GW}
(we will see some examples in Section \ref{s:furtherGW}), but
our primary interest in these notes resides in the latter.}
intersection numbers 
\begin{equation}
\label{eq:GW}
\int _{[\Mbar_{g,k} (X, \beta)] ^{\rm vir}} 
\ev_1^*(\gamma_1)\cup \ldots \cup \ev_k^*(\gamma_k),
\end{equation}
where:
$\gamma_1,\ldots,\gamma_k$ are cohomology classes in $H^*(X,\Z)$;
for all $i=1,\ldots,k$, $\ev_i$ is the \emph{evaluation map} at the
$i$-th marked point, \ie the map
$\Mbar _{g,k} (X,\beta) \to X$ defined by
$[f:C\to X,x_1,\ldots,x_k] \mapsto f(x_i)$;
$[\Mbar_{g,k} (X, \beta)] ^{\rm vir}$ is a rational homology class in
$H _{2 \vdim} \bigl(\Mbar_{g,k} (X, \beta), \Q \bigr)$,
called the \emph{virtual fundamental class},
where $\vdim$ is the expected (a.k.a.\ virtual) dimension of
$\Mbar_{g,k} (X, \beta)$.
The virtual fundamental class is the usual fundamental class when the
moduli space 
$\Mbar_{g,k} (X, \beta)$ has the expected dimension,
but in general it is given by an excess formula (it is the top Chern class
of the obstruction bundle when $\Mbar_{g,k} (X, \beta)$ is
non-singular).
Thus, the virtual fundamental class allows the computation of the
intersection product
$\ev_1^*(\gamma_1)\cup \ldots \cup \ev_k^*(\gamma_k)$
on $\Mbar_{g,k} (X, \beta)$ ``as if the latter were equidimensional of
the expected dimension''. 
Note that, by definition,
the integral \eqref{eq:GW} is $0$ if the degree of
the integrand does not match the dimension of the virtual fundamental
class. 

Typically, the cohomology classes $\gamma_1,\ldots,\gamma_k$ are
the Poincaré duals of algebraic cycles $\Gamma_1,\ldots,
\allowbreak\Gamma_k$ on
$X$; in this case, the condition that the degrees of
$\ev_1^*\gamma_1,\ldots, \ev_k^*\gamma_k$ sum up to
\sloppy $2 \vdim \Mbar_{g,k} (X, \beta)$
is equivalent to the equality
\begin{equation*}
\sum\nolimits _{i=1} ^k \bigl( \codim_X (\Gamma_i)-1 \bigr)
= \expdim \Mbar_{g,0} (X, \beta),
\end{equation*}
which means that the incidence conditions imposed by
$\Gamma_1,\ldots,\Gamma_k$ to genus $g$ curves in the class $\beta$
are expected to define a finite number of curves. Then, under
suitable transversality assumptions, and provided the moduli space
$\Mbar_{g,k} (X, \beta)$ (or equivalently $\Mbar_{g,0} (X, \beta)$)
has the expected dimension, the Gromov--Witten invariant \eqref{eq:GW}
gives the number of genus $g$ curves in the class $\beta$ (interpreted
as stable maps, and counted with multiplicities) which pass through
the cycles $\Gamma_1,\ldots,\Gamma_k$.
We will be mainly concerned in this text with the case when all
$\Gamma_i$'s are 
points, which is the only relevant case when $X$ is a surface.

% \par
% {\color{gray}
% I refer to
% \verb.{filippo-chap}. for a short introduction to Gromov--Witten theory
% at the same level as the present set of notes.
% }

\paragraph{Terminology and conventions}
We always work over the field of complex numbers.

Let $C$ be a curve. Its arithmetic genus, denoted by $p_a(C)$, is
the integer $1 - \chi(\O _C)$.
If $C$ is reduced, its geometric genus is
the arithmetic
genus of its normalization, and is denoted by
 $p_g(C)$.
When I write 'genus', this means 'geometric genus'.

A reduced curve $C$ is \emph{immersed} when the differential of
its normalization map is everywhere non-degenerate.
Concretely this means that $C$ has no cuspidal points; it may have
however points of any multiplicity, and non-ordinary singularities
(\eg a tacnode, \ie a point at which there are two smooth local
branches tangent one to another).
A \emph{node} is an ordinary double point.

A $K3$ surface $S$ is a smooth surface with trivial canonical bundle
and vanishing irregularity
(\ie $q(S)=h^1(S,\O_S)=0$); we may occasionally qualify as $K3$ a
surface with canonical singularities, the minimal smooth model of
which is a smooth $K3$ surface.
Let $p$ be a positive integer.
A $K3$ surface of genus $p$ is a pair
$(S,L)$, where $S$ is a $K3$ surface and $L$ an effective line
bundle on $S$, such that $L^2 = 2p-2$
(in particular, the $K3$ surface $S$ is algebraic). 
Under these assumptions, the complete linear system $|L|$ has
dimension $p$, and its general member has arithmetic genus $p$
(it is smooth if $|L|$ is free of fixed components).
The pair $(S,L)$ is \emph{primitive} if the line bundle $L$ is
indivisible, \ie there is no line bundle $L'$ on $S$ such that 
$L \cong (L') ^{\otimes m}$ for some integer $m>1$.

% By a smooth \emph{primitive} $K3$ surface of genus $p$, we mean a pair
% $(S,L)$ where $S$ is a smooth $K3$ surface, and $L$ an effective and
% \emph{indivisible} line bundle on $S$ such that $L^2 = 2p-2$.
% Then the complete linear system $|L|$ has dimension $p$, and its
% general member is a smooth curve of genus $p$.
% (We keep the letter $g$ for the geometric genus of (usually singular)
% curves $C$ in the linear system $|L|$).

In the notation of \ref{p:GW}, we write $\Mbar_{g}(X,\beta)$ for
$\Mbar_{g,0}(X,\beta)$. 
If $S$ is a surface equipped with an effective line bundle $L \to S$,
we write $\Mbar_{g,k}(X,L)$ for $\Mbar_{g,k}(X,\beta)$ where $\beta$
is the homology class of the members of $|L|$.


\paragraph{}
\label{p:discrep}
Let $(S,L)$ be a $K3$ surface of genus $p$.
Members of $|L|$ with exactly $\delta$ nodes as singularities have
geometric genus $p-\delta$, and are expected to fill up a locus of
codimension $\delta$ in $|L|$.
For this reason (and because $|L|$ has dimension $p$), the locus of
genus $g$ curves in $|L|$ has expected dimension $g$;
note that this does {not} match with the virtual dimension 
\eqref{eq:vdim0} of
$\Mbar_{g}(S,L)$,
see \ref{p:vanish}.
One can actually prove that this is indeed the correct dimension, and
that the locus of genus $g$ curves is equidimensional (see
\cite[\S~4.2]{DS15-10}). This implies that for a general set of $g$
points $x_1,\ldots,x_g \in S$, there is a finite number of genus $g$
curves in $|L|$ passing through all points $x_1,\ldots,x_g$,
by Kleiman and Piene's little lemma
\cite[Lemma \tref{lem:myfav}]{14.th-vainsencher}.


\paragraph{Acknowledgements}
I thank Jim Bryan and Rahul Pandharipande for patiently answering my
naive questions, and Yifan Zhao for his observations and help on
Section \ref{s:FGV-mult}.



\section{Rational curves in a primitive class}
\label{S:YZ}

In this section we discuss the following result, proved by Beauville
\cite{beauville-counting}
following a strategy proposed by Yau and Zaslow \cite{YZ}.
This strategy was inspired by physics; it is an
elaboration of the elementary argumentation 
using Euler numbers presented in Section~\ref{s:pencil}. 

\begin{theorem}[Yau--Zaslow, Beauville]
\label{T:YZ}
Let $(S,L)$ be a smooth primitive $K3$ surface of genus $p_0$,
and assume that $\Pic (S) = \Z \, L$.
Then there is a finite number $N ^{p_0}$ of rational curves in the complete
linear system $|L|$, and it is determined by the formula
\begin{align}
\label{eq:YZ}
1+ \sum _{p=1} ^{+\infty} N ^p q^p
\ &= \ \prod_{n = 1} ^{+\infty} \frac 1 {(1-q^n) ^{24}} \\
\notag &= \ 1 +24q +324q^2 +3200q^3 + \cdots
\end{align}
\end{theorem}

As one may expect, the number $N ^{p_0}$ is the number of rational
curves counted with appropriate multiplicities. As we shall see, the
multiplicity of an integral rational curve $C$ is the
topological Euler number $e(\bar JC)$ of its compactified Jacobian,
and it depends only on the equisingularity class of its
singularities.
It may be explicitly computed in many cases; in particular, it is $1$
whenever the curve is immersed. 
For a very general $(S,L)$, all rational curves in $|L|$ are 
nodal by \cite{chen-10}, hence in this case all rational curves count
with multiplicity one.

The assumption that $\Pic (S) = \Z \, L$ is made to ensure that
{all} members of $|L|$ are integral curves.
While it may be possible to adapt the arguments given by Beauville
and Yau--Zaslow to the case when some members of
$|L|$ are reducible but reduced,
the presence of non-reduced members of $|L|$ poses problems of a
different nature, see Section~\ref{S:BPS}.

Theorem~\ref{T:YZ} is a particular case of the more general result
discussed in Section~\ref{S:BL}. We will recall there the relevant
facts from the theory of modular forms needed to explore the modular
aspects of formula \eqref{eq:YZ}, and give more values of $N ^p$ for
small $p$.


\subsection{An elementary topological counting formula}
\label{s:pencil}

Let $X$ be a complex compact manifold and $\ff$ a $1$-dimensional
family of divisors of $X$, such that the general member of $\ff$ is
smooth and $\ff$ has no fixed part.
It is possible to count the number of singular members of $\ff$ using
the topological formula stated in Lemma~\ref{l:pencil} below.

\paragraph{Euler number}
\label{p:euler}
Let $X$ be a topological space. The
\emph{(topological) Euler number} of $X$ is
\begin{equation*}
e(X) = \sum _i (-1)^i \dim H_c^i(X,\Z),
\end{equation*}
where the subscript $c$ means cohomology with compact support.

If $X$ is compact and $F \subset X$ is a closed subset,
then the following \emph{additivity formula} holds:
\begin{equation*}
e(X) = e(X-F) + e(F).
\end{equation*}
It follows from the
long exact sequence 
\[
\cdots \to
H^i _{c} (X-F,\Z) \to
H^i (X, \Z) \to
H^i (F, \Z) \to
H^{i+1} _{c}(X-F, \Z) \to
\cdots
\]
see \cite[Théorème 4.10.1]{godement}.

\begin{lemma}
\label{l:pencil}
Let $f:X \to C$ be a surjective morphism from a complex compact manifold
onto a smooth curve. 
One has
\begin{equation}
\label{eq:pencil}
e(X)=
e(F_{\rm gen}) \, e(C)+
\sum_{y\in \Disc (f)}\bigl(e(F_y)-e(F_{\rm gen})\bigr),
\end{equation}
where $F_{\rm gen}$ is the fibre of $f$ over a general point of $B$,
and for all $y\in B$, $F_y$ is the fibre over $y$;
$\Disc (f) \subset C$ is the set of points above which $f$ is not smooth.
\end{lemma}

\begin{proof}
Set $U = X - \bigcup _{y \in \Disc (f)} F_y$. Then
$f : U \to C-\Disc (f)$ is a topological fibre bundle, hence
\[
e(U) = e(C-\Disc (f)) \, e(F_{\rm gen}).
\]
Now, by the additivity formula,
\[
  e(X) = e(U) + \sum_{y\in \Disc (f)} e(F_y)
  \Et
  e(C-\Disc (f)) = e(C) - \sum_{y\in \Disc (f)} 1,
\]
and Formula \eqref{eq:pencil} follows.
\end{proof}


\paragraph{}
The upshot of Lemma \ref{l:pencil} is that the number of singular
fibres of $f:X \to C$ is
$e(X) - e(F_{\rm gen}) \, e(C)$, provided each singular fibre $F_y$ is
counted with multiplicity $e(F_y) - e(F_{\rm gen})$.
When $X$ is a surface and the schematic fibre over $y$ is reduced, the
difference $e(F_y)-e(F_{\rm gen})$ is determined by the singularities
of $F_y$, as we shall now explain.

Let $D$ be a reduced projective curve,
$\Sigma$ its singular locus,
$\nu: \bar D \to D$ its normalization,
and $\bar \Sigma = \nu ^{-1} (\Sigma)$.
Since $\bar D - \bar \Sigma$ and $D-\Sigma$ are isomorphic one has,
by the additivity formula,
\begin{equation}
\label{eq:eDbarD}
\begin{aligned}
e(D) &= e (D-\Sigma) + e(\Sigma)
 \\
&= e (\bar D- \bar \Sigma) + e(\Sigma)
% + e(\bar \Sigma) -  e(\bar \Sigma)
 \\
&= e (\bar D- \bar \Sigma)  + e(\bar \Sigma) + e(\Sigma)
 -  e(\bar \Sigma)
= e(\bar D) - \bigl( \Card (\bar \Sigma)
- \Card (\Sigma) \bigr).
%\label{chi-tilde-et-non}
\end{aligned}
\end{equation}

Now, let $f: S \to C$ be a surjective morphism from a smooth projective
surface to a smooth curve, and consider a point $y \in C$ such that
the schematic fibre $F_y$ is reduced. Then the curve $F_y$ has the
same arithmetic genus as the general fibre $F _{\rm gen}$,
and $\bar F_y$ is a smooth curve of genus $p_a(F_\gen)-\delta$,
where $\delta = p_a(F_y)-p_g(F_y)$ is the sum of the
$\delta$-invariants of all singularities of $F_y$.
Therefore,
\begin{equation*}
  e(\bar F_y) = 2-2(p_a(F_\gen)-\delta)
  = e(F_{\rm gen}) + 2\delta,
\end{equation*}
hence
\begin{equation*}
e(F_y)-e(F_{\rm gen}) = 2\delta - \bigl( \Card (\bar \Sigma_y)
- \Card (\Sigma_y) \bigr)
\end{equation*}
by \eqref{eq:eDbarD}.
This proves the following.

\begin{lemma}
\label{l:pencil-mult}
In the above notation, the multiplicity with which the fibre $F_y$
is counted in Formula \eqref{eq:pencil} is a sum of local
multiplicities computed at the singular points of $F_y$, namely
\begin{equation*}
e(F_y)-e(F_{\rm gen}) = \sum _{x \in\Sing F_y}
\left( \delta(F_y,x) -\# \Bigl(
\begin{matrix}
\text{local branches} \\ 
\text{of $F_y$ at $x$}
\end{matrix}
\Bigr)
+1
\right).
\end{equation*}
\end{lemma}

\noindent
This gives for example the local multiplicity $1$ for a node,
$2$ for an ordinary cusp, $3$ for a tacnode, and $4$ for an ordinary
triple point.


\paragraph{Application to $K3$ surfaces of genus one}
\label{p:ellK3}
Let $(S,L)$ be a primitive $K3$ surface of genus one.
If $\Pic(S)=\Z\,L$, then $|L|$ is a
base-point-free pencil of elliptic curves, and all its members are
reduced since $L$ is not divisible. 
All $K3$ surfaces $S$ have $e(S)=24$,
and smooth elliptic curves have Euler number $0$.
Thus, it follows from
formula \eqref{eq:pencil} that $|L|$ has $24$ singular members,
counted with the multiplicity given in Lemma~\ref{l:pencil-mult}.
This agrees with Theorem~\ref{T:YZ}.


\paragraph{}
Finally,
if $\ff$ is a $1$-dimensional
family of divisors on a compact complex manifold $X$, free of fixed
component and such that the general member of $\ff$ is
smooth, in order to find the number of singular members of $\ff$ one
may consider the minimal smooth blow-up $\tilde X \to X$ such that the
proper transform of $\ff$ is base-point-free;
then there is a regular map $\tilde X \to \ff$, the fibres of which are
exactly the members of $\ff$, and one may apply Lemma \ref{l:pencil}
to this fibration.


\subsection{Proof of the Beauville--Yau--Zaslow formula}
\label{s:YZ-proof}

In this section, we outline the proof of Theorem \ref{T:YZ}.
Let $p$ be a positive integer, $(S,L)$ a smooth primitive $K3$
surface of genus $p$, and $\fL$ the complete linear system
$|L|$. We assume that all members of $\fL$ are integral.

We let $\cC$ be the
universal curve over $\fL$, and consider the component
\begin{equation*}
\pi: \cJac^p \cC \to \fL
\end{equation*}
of the compactified Picard scheme of the family $\cC \to
\fL$ which parametrizes pairs $(C,M)$ made of a member $C$ of $\fL$ and
a rank $1$, torsion-free, coherent sheaf $M$ of degree $p$ on $C$.
For all $[C] \in \fL$,
the fibre $\pi^{-1}([C])$ is the compactified Jacobian $\bar J^p C$ of
$C$. 
The total space $\cJac^p \cC$ is a projective variety of dimension
$2p$, which we will call the universal compactified Jacobian.

\begin{claim}
\label{p:YZ-concl}
The Euler number 
$e(\cJac^p \cC)$ is the number of rational curves in $\fL$, where each
rational curve $C$ is counted with multiplicity $e(\bar J^p C)$.
\end{claim}

\begin{proof}
The claim relies on the fact
that for all $[C] \in \fL$,
the fibre
$\pi^{-1}([C]) = \bar J^p C$ 
has non-vanishing Euler number if and only if $C$ is rational,
see Propositions~\ref{P:e-vanish} and \ref{P:e-rat} in
Section \ref{s:cpct-Jac} below.

The rest is essentially an elaboration of Lemma~\ref{l:pencil} and its
proof.
There exists a stratification $\fL = \coprod_\alpha
\Sigma_\alpha$ by locally closed subsets such that $\pi$ is
topologically locally
trivial over each stratum $\Sigma_\alpha$ \cite{verdier-whitney}.
Then,
\begin{equation}
\label{eq:e-compact-J}
e(\cJac^p \cC) = 
\sum _\alpha
e \bigl( \pi^{-1}(\Sigma_\alpha) \bigr)
\end{equation}
by the additivity formula, and for each $\alpha$ one has
\[
e \bigl( \pi^{-1}(\Sigma_\alpha) \bigr) = 
e(\Sigma _\alpha) \times e(\bar J_\alpha)
\]
where $\bar J_\alpha$ stands for the fibre of $\pi$ over any point in the
stratum $\Sigma _\alpha$. 
Since $e(\bar J^p C)=0$ if the curve $C$ is not
rational, the sum in \eqref{eq:e-compact-J} reduces to the sum over
all $\alpha$ such that the curves parametrized by the stratum
$\Sigma_\alpha$ are rational.
Now, the union of these strata is a finite set
(see, \eg \cite[Prop.~(4.7)]{DS15-10}), which we shall denote by
$\fL_{\rm rat}$, and we finally find
\begin{equation}
\label{eq:e-count}
e(\cJac^p \cC)
= \sum _{[C] \in \fL_{\rm rat}} e(\bar J^p C),
\end{equation}
which proves the claim.
\end{proof}


Let $S^{[p]}$ be the component of the Hilbert scheme of $S$ parametrizing
$0$-dimensional subschemes of length $p$. It is a smooth
Hyperkähler variety of dimension $2p$, see \cite{beauville-c1}.


\begin{claim}
\label{cl:cJac-Hilb-Euler}
The universal compactified Jacobian $\cJac^p \cC$
and the Hilbert scheme $S^{[p]}$ have the same Euler numbers, given by
Formula \eqref{eq:YZ}.
\end{claim}

\begin{proof}
First, the universal compactified Jacobian $\cJac^p \cC$
is smooth and Hyperkähler,
as noted in \cite[Example~0.5]{mukai-symplectic},
because it is a
connected component of the moduli space of simple sheaves on the $K3$
surface $S$.
It is sometimes called the Beauville--Mukai system.

Next, let us prove that $\cJac^p \cC$ and $S^{[p]}$ are birational.
This will imply, by a theorem of Huybrechts
\cite[p.~65]{huybrechts-diffeo},
that $\cJac^p$ and $S^{[p]}$ are 
deformation equivalent, hence share the same Betti
numbers, so that $e(\cJac^p) = e(S^{[p]})$.

There is an open subset $U \subseteq \cJac^p \cC$ whose points are
pairs $(C,M)$ such that $C$ a smooth (genus $p$) member of $\fL$ and
$M$ is a 
non-special, degree $p$, line bundle on $C$.
For such a pair one has $h^0(C,M)=1$, and
the unique divisor $D$ in the complete linear system $|M|$ may be seen
as a point of $S^{[p]}$: this gives a regular map
$U \to S^{[p]}$.
On the other hand, the fact that $h^1(C,\O_C(D))=0$ implies by
geometric Riemann--Roch that $D$ spans the whole space in the
canonical embedding of $C$, hence
$C$ is the only member of $\fL$ that contains $D$.
Therefore, the map $(C,M)\in U \mapsto D$ is injective, and this ends
the proof of the birationality of $\cJac^p \cC$ and $S^{[p]}$.


Finally, the fact that $e(S^{[p]})$ is the coefficient
of $q^p$ in
the Fourier expansion of $\prod _{n=1}^\infty (1-q^n)^{-24}$ as in 
\eqref{eq:YZ}
follows from the computation by Göttsche of the Betti and
Euler numbers of $S^{[p]}$ for any smooth, complex, projective surface
\cite{goettsche-betti-nbrs}.
This computation is based on the idea of using the Weil conjectures
(proved by Deligne) to translate the question into that of counting the
points of $S^{[p]}$ over finite fields.
\end{proof}

\noindent
Claims \ref{p:YZ-concl} and \ref{cl:cJac-Hilb-Euler} together imply
Theorem~\ref{T:YZ}.


\subsection{Compactified Jacobian of an integral curve}
\label{s:cpct-Jac}

Let $C$ be  an integral curve.
We now turn to the study of the Euler number of the compactified
Jacobian $\bar J^d C$.
% which parametrizes rank one, torsion free,
% coherent sheaves of degree $d$ on $C$. 
We will in particular prove some results used in the proof of
Claim \ref{p:YZ-concl} in Section~\ref{s:YZ-proof}.
As is well-known, the choice of an invertible sheaf of degree $d$
on $C$ induces an isomorphism between $\bar J^d C$ and $\bar J C =
\bar J^0 C$, so we will actually consider the latter variety. 

\begin{proposition}
\label{P:e-vanish}
If $C$ is an integral curve of positive geometric genus, then 
$e(\bar JC)=0$.
\end{proposition}

\begin{proof}
There is an exact sequence 
\begin{equation*}
0 \to H \to JC \to J\tilde C \to 0
\end{equation*}
where $\tilde C$ is the normalization of $C$,\footnote
{exceptionally, I do not use the notation $\bar C$ in order to avoid
unpleasant confusions between $\bar JC$ and $J\bar C$}
$J$ denotes the Jacobian $\Pic^0$,
and $H$ is a product of copies of $(\C,+)$ and $(\C^*,\times)$
(see, \eg \cite[Thm.~7.5.19]{qing-liu}).
Since $H$ is divisible, the sequence  splits as an exact sequence of
Abelian groups, hence
$JC = J\tilde C \times H$.
Since $J\tilde C$ is a positive dimensional torus,
for all positive integers $n$, there exists
an order $n$ group
$G_n$ which is a subgroup of both $JC$ and $J\tilde C$.

Then, \cite[Lemma~2.1]{beauville-counting} tells us that for all $M
\in G_n$ and $\cF \in \bar JC$, the two sheaves $\cF$ and $\cF
\otimes M$ are {not} isomorphic.
Thus $G_n$ acts freely on $\bar JC$, hence $n$ divides
$e(\bar JC)$. Since this is true for all $n$, we conclude that $e(\bar
JC)=0$.
\end{proof}

We need the following local construction 
(\cf \cite[\S 3.6]{beauville-counting} and the references therein)
in order to make
$e(\bar JC)$ explicit for a rational curve $C$.

\paragraph{}
\label{p:local-e}
Let $(C,x)$ be a germ of curve which we assume to be unibranch
(see \ref{p:unibranch}
below), and let
$\tilde C$ be
the normalization of $C$; there is only one point in the preimage of
$x$, which we call $x$ as well.
Set $\delta_x= \dim \O_{\tilde C,x} / \O_{C,x}$ (this is the number by
which a singularity equivalent to $(C,x)$ makes the geometric genus
drop), and let $\bc'_x$ be the ideal 
$\O_{\tilde C} (-2\delta\cdot x)$.\footnote
{we reserve the notation $\bc_x$ for the conductor ideal
  (see \cite{02.edoardo}), which contains
$\bc'_x$}
We shall
consider the two finite-dimensional algebras $A_x:= \O_{C,x}/\bc'$ and
$\tilde A_x:=  \O_{\tilde C,x}/\bc'$.

Let $\bG_x$ be the closed subvariety of the
Grassmannian $\bG (\delta_x, \tilde A_x)$ parametrizing
those codimension $\delta_x$ subspaces of $\tilde A_x$ that are also
sub-$A_x$-modules of $\tilde A_x$;
$\bG_x$ may also be seen as the variety parametrizing codimension
$\delta_x$ sub-$\O_{C,x}$-modules of $\O _{\tilde C,x}$. It only
depends on the completion $\hat \O _{C,x}$, hence only on the analytic
type of the singularity $(C,x)$.

\paragraph{}
\label{p:unibranch}
A curve is \emph{unibranch} if its normalization is a
homeomorphism, or equivalently if it is everywhere analytically
locally irreducible. 
All curves $C$ have a \emph{unibranchization} 
$\breve\nu: \breve C \to C$: this is the unique partial normalization
of $C$ such that $\breve C$ is unibranch, and such that
all others partial normalizations $\nu':C' \to C$ with $C'$ unibranch
factor through $\breve \nu$. 
\par If $C$ is a unibranch curve with singular locus $\Sigma
\subset C$, the product $\prod _{x \in \Sigma} \bG_x$ parametrizes
sub-$\O_C$-modules $\cF \subset \O _{\tilde C}$ such that 
$\dim \O _{\tilde C,x} / \cF_x = \delta_x$ for all $x$. Such an $\cF$
enjoys the property that $\chi (\cF) = \chi (\O_C)$, which implies
$\cF \in \bar JC$. This defines a morphism
\begin{equation*}\textstyle
\epsilon: \prod _{x \in \Sigma} \bG_x \to \bar JC.
\end{equation*}
Part (ii) in the following statement is proved by showing that 
$\epsilon$ is a
homeomorphism if $C$ is rational, though in general not an
isomorphism.
% Note that since $\bG_x$ is a point when $(C,x)$ is a smooth curve
% germ, one has $\prod _{x \in \Sigma} e(\bG_x) = 
% \prod _{x \in C} e(\bG_x)$.

\begin{proposition}
\label{P:e-rat}
{\normalfont
(i) \cite[Prop.~3.3]{beauville-counting}}
If $C$ is an integral curve, then 
$e(\bar JC) = e(\bar J\breve C)$.\\
{\normalfont
(ii) \cite[Prop.~3.8]{beauville-counting}}
If $C$ is a unibranch rational curve with singular locus
$\Sigma$, then 
$e(\bar JC) =  \prod _{x \in \Sigma} e(\bG_x)$.
\end{proposition}


By (i), one has $e(\bar JC) =1$ for an
immersed rational curve $C$
($C$ is immersed if all its analytic local branches are smooth,
equivalently if the unibranchization $\breve C$ is smooth).
If $C$ is not immersed, then $e(\bar JC) = e(\bar J\breve C)$ and the
latter number is computed by (ii);
it follows from Theorem \ref{T:fgv1} in the next subsection that
this number is positive if $C$ is a rational curve lying on a smooth
surface. 

Part (ii) also shows that
for all rational curves $C$ (unibranch or not, thanks to (i)),
$e(\bar JC)$ is entirely determined by the singularities of $C$.
In fact it only depends on their topological types
if $C$ has planar singularities,
see Corollary \ref{cor:top-ct} below.


\begin{example}[{\cite[\S~4]{beauville-counting}}]
If $(C,x)$ is the germ of curve given by the equation $u^p+v^q=0$ at
the origin in the affine plane, with $p$ and $q$ relatively prime,
then
\begin{equation}
\label{ex:up+vq}
e(\bG_x) = \frac 1 {p+q} \binom {p+q} p.
\end{equation}
Formula \eqref{ex:up+vq} also gives $e(\bG_{x'})$ for all singularities
$(C',x')$ equisingular to $(C,x)$ by the aforementioned
Corollary \ref{cor:top-ct}.

In particular, 
$e(\bG_x) = \ell+1$ for the cuspidal singularity defined by
the equation $u^2+v^{2\ell+1}=0$, \ie
for an $A_{2\ell}$-double point;
on the other hand $A_{2\ell+1}$-double points are immersed, hence
$e(\bG_x) = 1$ for them.
Using Proposition~\ref{P:e-rat}, (i), to the effect that the local
contribution $e(\bG_x)$ of a germ $(C,x)$ is the product of the local
contributions of all analytic local irreducible branches of $(C,x)$,
Formula
\eqref{ex:up+vq} is enough to determine the local contribution
$e(\bG_x)$ of any
simple curve singularity, see \cite[Prop.~4.5]{beauville-counting}.
\end{example}


\paragraph{Remark} 
\label{rk:red-in-pencil}
The fact that all immersed rational curves count with multiplicity one
seems to disagree with the
results of Section~\ref{s:pencil}, see in particular
Lemma~\ref{l:pencil-mult}. 
%computation of \ref{p:ellK3}.
However, if $|F|$ is a complete pencil of
elliptic curves, the assumption that all curves in $|F|$ are integral
implies that all rational curves in $|F|$ are curves of
arithmetic genus $1$ with either a node or an ordinary cusp as their
unique singular point,
and in this case the two multiplicities predicted by
Proposition \ref{P:e-rat}
and Lemma~\ref{l:pencil-mult}
do agree.


\paragraph{Remark}
\label{rk:rather-surp}
Returning to the case of a $p$-dimensional linear system $\fL$ with
all members integral, Beauville
%makes a remark similar to \ref{rk:red-in-pencil},
deems ``rather surprising'' the fact that
``some highly singular [immersed] curves count with multiplicity
one'', and considers the case $p=2$ to provide a confirming example.

\smallskip
\subparagraph{}
In hindsight, 
a good conceptual explanation comes from the fact 
that the numbers $N^p$ should be seen as counting stable
maps rather than embedded curves, since stable maps don't make any
difference between nodal and arbitrary immersed curves:
if $p$ is a singular point of a curve $C$ and $p'$ is a point of the
normalization $\tilde C$ mapping to $p$, analytically locally at $p'$
one does not see how the local branch of $C$ at $p$ corresponding to
$p'$ intersects the other local branches (one does see however if this
branch of $C$ is singular, by looking at the
differential of the map $\tilde C \to C$).
This heuristic argument is confirmed by Theorem \ref{T:fgv2b} in the
next subsection,
see also Lemma \ref{l:enum}.


\smallskip
\subparagraph{}
\label{rk:rather-surp:EG}
Another comforting observation is that the equigeneric
%locus in the semi-universal
deformation space of an immersed singularity is
smooth, as we shall see in
\ref{p:imm-EG} in the next subsection.
Indeed, let $C$ be a rational member of $\fL$.
There exists an analytic
neighbourhood of $[C]$ in $\fL$ and a map $\phi$ from $U$ to the
semi-universal deformation space $B$ of the singularities of $C$, which
encodes the singularities of the curves neighbouring $C$ in $\fL$.
Then, the locus of rational curves in $U$ is the inverse image by
$\phi$ of the equigeneric locus $\EG(C)$ in $B$,
hence it is reasonable to imagine that the
multiplicity of $C$ in the count of
rational curves is the multiplicity of the $0$-cycle
$\phi^* \EG(C)$ at the point $[C] \in U$. The fact that
rational curves in $\fL$ are finitely many implies as in
\ref{p:discrep} that the intersection $\phi(U) \cap \EG(C)$ has the
expected dimension.
If we assume furthermore that $\phi$ is an immersion and $\phi(U)$
intersects $\EG(C)$ transversely, then the multiplicity of
$\phi^* \EG(C)$ at $[C]$ equals the multiplicity of the origin of $B$
as a point of $\EG(C)$.

In the upshot, it is plausible that a rational curve counts with
multiplicity equal to the multiplicity of the origin in the
equigeneric deformation space of its singularities.
Since the latter
multiplicity is one if all singularities of $C$ are immersed, it is
plausible that any immersed rational curve counts with multiplicity one.
In fact, we shall see in Section \ref{s:FGV-mult} that things happen
exactly as described above.




% In the next subsection we will see two results of Fantechi, Göttsche,
% and van Straten which extend and confirm the considerations of
% %\ref{rk:red-in-pencil} and
% Remark~\ref{rk:rather-surp} above.


\subsection{Two fundamental interpretations of the
multiplicity}
\label{s:FGV-mult}

We now conclude Section \ref{S:YZ} by stating two enlightening
geometric 
interpretations of the local multiplicities $e(\bG_x)$ defined in the
previous subsection,
due to Fantechi, G\"ottsche and van Straten \cite{fgv}.

In the present subsection we only consider \emph{planar} curve
singularities $(C,x)$, \ie singularities that may be realized by the
germ of a plane curve. All singularities occuring on a curve that lies
on a smooth surface are of this kind.

\begin{theorem}[{\cite[Thm.~1]{fgv}}]
\label{T:fgv1}
Let $(C,x)$ be a reduced, planar, curve singularity, and let
$\bG_x$ be as in \ref{p:local-e}.
Then the topological Euler number $e(\bG_x)$ equals the multiplicity
at the point $[(C,x)]$ of the equigeneric locus $\mathrm{EG} (C,x)$ in
the semi-universal deformation space of the singularity $(C,x)$.
\end{theorem}

Recall that the \emph{equigeneric locus} $\mathrm{EG} (C,x)$ is
defined as the reduced subscheme of the semi-universal deformation
space of the singularity $(C,x)$ supported on those points
corresponding to singularities with the same $\delta$-invariant as
$(C,x)$.
In practice this is the closure of
the locus along which the singularity deforms to
$\delta$ nodes, where $\delta$ is the number by which the singularity
makes the geometric genus drop.
See, \eg \cite{02.edoardo} for more details.

Together with Proposition~\ref{P:e-rat},
Theorem \ref{T:fgv1} implies that for a rational,
integral, curve $C$ with only planar singularities, the
Euler number $e(\bar JC)$ of the compactified Jacobian of
$C$ equals the multiplicity at the point $[C]$ of the equigeneric
stratum $\mathrm{EG}(C)$ in a semi-universal deformation space of
the singularities of $C$.
See \ref{rk:rather-surp:EG} above for a discussion of why this
provides a
reasonable notion of multiplicity for $C$ in a count of rational
curves.

\medskip
Theorem \ref{T:fgv1} has been generalized by Shende
\cite{shende-strata}, to the effect that
the multiplicity at $[C]$
of all $\delta$-constant strata in a semi-universal deformation space
of the singularities of $C$
are determined by the Euler numbers of the Hilbert schemes of
points on $C$
(for a curve $C$ of arbitrary genus).

On the other hand, Maulik \cite{maulik-homfly} has proved that the
Euler numbers of the Hilbert schemes of points
$(C,x)^{[n]}$ of a planar curve singularity only depend on the
topological type of the singularity. This implies the following.

\begin{corollary}[see {\cite[\S~6.5]{maulik-homfly}}]
\label{cor:top-ct}
Let $(C,x)$ be a reduced, planar, curve singularity.
The multiplicities at the point $[(C,x)]$ of the $\delta$-constant
(a.k.a.\ constant genus) strata of 
the semi-universal deformation space of the singularity $(C,x)$ only
depend on the topological type (or equisingularity class) of $(C,x)$. 
\end{corollary}



\paragraph{}
\label{p:imm-EG}
As a corollary of Theorem~\ref{T:fgv1} and Proposition~\ref{P:e-rat},
one obtains that if $(C,x)$ is an immersed planar curve singularity,
then the equigeneric locus $\EG(C,x)$ in the space of semi-universal
deformations is smooth at the point $[(C,x)]$.
Indeed, note that for all reduced plane curve singularities $(C,x)$, there
exists a rational curve $\tilde C$ with $(C,x)$ as its only singularity
(this follows for instance from \cite{morelli}),
and then one has $e(\bG_x)= e(\bar J \tilde C)$.

In fact the converse holds as well, \ie
for a reduced planar curve singularity $(C,x)$, the equigeneric locus  
$\EG(C,x)$ is smooth at the
point $[(C,x)]$ if and only if $(C,x)$ is immersed,
see \cite[Proposition (4.17), (2)]{diaz-harris}.


\bigskip
Now let us turn to the second interpretation of the multiplicity
$e(\G_x)$, or rather of
$e(\bar JC) =  \prod _{x \in \Sigma} e(\bG_x)$.
It tells us that what the
Yau--Zaslow formula~\eqref{eq:YZ} really computes is the numbers of
genus $0$ stable maps realizing primitive classes on $K3$ surfaces.
Recall that if $C$ is an integral curve of geometric genus $g$
which is a subvariety of a complex variety $X$, then
$\Mbar_g (X,[C])$ is the space of genus
$g$ stable maps with target $X$ realizing the homology class $[C] \in
H_2(C,\Z)$. 

\begin{theorem}[{\cite[Thm.~2]{fgv}
  and \cite{yifan_zhao}}]
\label{T:fgv2b}
Let $C$ be an integral rational curve contained in a smooth $K3$
surface $S$. Then the topological Euler number $e(\bar JC)$ equals the
length of the space of stable maps $\Mbar_0 (S,[C])$ at the closed
point corresponding to the normalization of $C$.
\end{theorem}

I have been informed by Yifan Zhao that he has found a problem in the
proof of \cite[Thm.~2]{fgv}, and will provide a corrected proof in the
upcoming \cite{yifan_zhao}; I refer to \cite{yifan_zhao} for the full
details.

Fantechi--G\"ottsche--van Straten first consider the space
$\Mbar_g (C,[C])$ of stable maps to $C$ itself which realize the
fundamental class $[C]$.
It is a $0$-dimensional scheme, which contains a single
closed point, corresponding to the normalization $\nu: \bar C \to C$.
If $C$ is an isolated, genus $g$ curve in a smooth manifold
$X$, then $\Mbar_g(C,[C])$ is a subscheme of $\Mbar(X,[C])$
and, at the normalization of $C$,
the length of the former scheme is a lower bound for the
length of the latter.

Now, in \cite[Thm.~2]{fgv} the authors claim that
for an integral projective curve $C$ of genus $g$ with planar
singularities, the length of  
$\Mbar_g (C,[C])$ equals the multiplicity at $[C]$ of the
semi-universal deformation space of the singularities of $C$.
However, \cite[\S 7.2.2]{oblomkov-yun} provides a counterexample,
namely a rational curve $C$ with planar singularities such that the
Euler number $e(\bar JC)$ is larger than the length of
$\Mbar_0 (C,[C])$
(as we have seen, since $C$ is rational, $e(\bar JC)$
equals the multiplicity at $[C]$ of the
semi-universal deformation space).




\section{Curves of any genus in a primitive class}
%{Gromov--Witten invariants for $K3$ surfaces}
\label{S:GWK3}

\subsection{Reduced Gromov--Witten theories for $K3$
  surfaces}
\label{s:red-th}

\paragraph{A vanishing phenomenon}
\label{p:vanish}
It happens that all Gromov--Witten invariants of $K3$ surfaces are
trivial. The fundamental reason for this is that Gromov--Witten
invariants are deformation invariant (this is indeed a desirable
feature of any well-behaved counting invariants, and the very reason
why they are called invariants and not merely numbers, or integrals),
and all algebraic $K3$ surfaces deform to
non-algebraic ones, which in general do not contain any curve
at all.

Somewhat more concretely, the explanation is that the virtual and
actual dimensions of the moduli spaces of stable maps on $K3$ surfaces
do not match, as we already pointed out in \ref{p:discrep}.
Let
$S$ be a $K3$ surface, and $C \subset S$ an integral curve of
geometric genus $g$. Consider the stable map $f: \bar C \to S$
obtained by composing the normalization $\bar C \to C$ with the
inclusion $C \subset S$. The normal sheaf $N_f$ of $f$ is
isomorphic to the canonical  bundle $\omega _{\bar C}$, and therefore 
$h^0(N_f)=g$ and $h^1(N_f)=1$.
It follows that the virtual dimension of 
$\overline {M}_g(S,[C])$ is $g-1$, whereas the curve $C$ actually
moves in a $g$-dimensional family of curves of genus $g$ on $S$
(see \cite[\S~4.2]{DS15-10} for more details).
This implies that the Gromov--Witten invariant counting genus $g$
curves on $S$ passing through the appropriate number of points (namely
$g$) vanishes for mere degree reasons.
% The case $g=0$ is particularly striking; then the virtual dimension
% being $-1$ means that there should not be any rational curve at all on
% $S$.

\medskip
The following two paths have been successfully followed to circumvent
this issue, and define modified invariants for algebraic $K3$
surfaces which capture the relevant enumerative
information.

\paragraph{Invariants of families of symplectic structures
  {\normalfont \cite[\S~2--3]{BL}}%
}
\label{p:sympl}
This was chronologically the first workaround to be proposed, and it
enabled the counting of curves of any genus in a primitive class on a
$K3$ surface reported on in Section \ref{S:BL} below.

Let $S$ be a polarized $K3$ surface.
 The idea here is really to take into account the existence of
non-algebraic deformations of $S$. To this effect, instead of counting
curves directly on $S$, one counts curves in a family of Kähler
surfaces defined over the $2$-sphere $\mathbf{S}^2$, canonically
attached to $S$, and in which roughly speaking $S$ is the only one to
be algebraic, so that all the curves we count are actually
concentrated on $S$.
\par This family of Kähler surfaces is the twistor family of $S$
(\cf \cite[p.~124]{palaiseau}): the
polarization on $S$ determines a Kähler class $\alpha$, and Yau's
celebrated theorem asserts that there is a unique Kählerian metric $g$
in $\alpha$ with vanishing Ricci curvature.
Then the holonomy defines an action of $\bf{H}$ (the field of
quaternion numbers) on the holomorphic tangent bundle $TS$ by parallel
endomorphisms. The quaternions of square $-1$ define those complex
structures on the differentiable manifold $S$ for which the metric $g$
remains Kählerian. There is a $2$-sphere worth of such quaternions,
and it parametrizes the family we are interested in.

\paragraph{Reduced Gromov--Witten theory
  {\normalfont (\cite[2.2]{MP}, see also \cite{MPT})}%
}
\label{p:redGW}
In this second approach, the idea is to plug in the fact that, for a
stable map $f$ as in \ref{p:vanish}, the space $H^1(\bar C, N_f)$
although non-trivial does not contain any actual obstruction to deform
$f$ as a map with target $S$, following for instance Ran's results on
deformation theory and the semiregularity map. To this end, Maulik and
Pandharipande define a suitable perfect obstruction theory which they
dub \emph{reduced}, and which provides,
following the construction pioneered by Behrend and Fantechi,
a reduced virtual fundamental
class $[\overline{M}_g (S,\beta)] ^{\rm red}$,
for all integers $g \geq0$ and algebraic classes $\beta \in
H_2(S,\Z)$, 
which has the appropriate (real) dimension $2g$.
\par
This in turn gives reduced Gromov--Witten integrals, by replacing the
virtual fundamental class by its reduced version in the integral
\eqref{eq:GW}.
They are invariant under
\emph{algebraic} deformations of $K3$ surfaces.

\subsection{The G\"ottsche--Bryan--Leung formula}
%{Curves of any genus in a primitive class}
\label{S:BL}

In this subsection, I discuss a result of Bryan and Leung \cite{BL}
giving the number of curves in a primitive linear system on a $K3$
surface that have a given genus and pass through the appropriate
number of base points.
The formula was conjectured by G\"ottsche \cite{goettsche-conj} as a
particular case of a more general framework,
see \cite{12.fra-goettsche}.

Let
\begin{equation*}
N^p_g := 
\int _{[\Mbar_{g,g} (S,L)] ^{\rm red}} \ev_1^* (\pt) \cup \cdots
\cup \ev_g^* (\pt)
\end{equation*}
be the reduced Gromov--Witten invariant counting curves
of genus $g$ in the linear system $|L|$ on a primitive
$K3$ surface $(S,L)$ of genus $p$
($\pt \in H^4(S,\Z)$ is the point class, and the $\ev_1, \ldots,
\ev_g$ are the evaluation maps 
$\Mbar_{g,g} (S,L) \to S$, as in \ref{p:GW}).
The following result tells us that these invariants do indeed count
curves. 

\begin{lemma}
\label{l:enum}
The invariants $N^p_g$ are strongly enumerative, in the following sense:
let $(S,L)$ be a very general primitive $K3$ surface of genus $p$;
then $N^p_g$ is the actual number of genus $g$ curves in $|L|$ passing
through a general set of $g$ points, all counted with multiplicity
$1$.
\end{lemma}

\begin{proof}
The key fact is that genus $g$ curves on a $K3$ surface move in
$g$-dimensional families, see \eg \cite[Prop.~(4.7)]{DS15-10};
for $g>0$, this implies by a deformation argument that the general
member of such a family is an immersed curve
\cite[Prop.~(4.8)]{DS15-10}. 
The same holds for $g=0$ by the more difficult result of Chen
\cite{chen-10}, which asserts that
all rational curves in $|L|$ are nodal
(this requires the very generality assumption).

Let ${\bf x}=(x_1,\ldots,x_g)$ be a general (ordered) set of $g$ points
on $S$. The invariant $N^p_g$ may be computed by integration against a
virtual class on the so-called cut-down moduli space 
$\Mbar(S,\bx) \subset \Mbar_{g,g}(S,L)$,
consisting of those genus $g$ stable
maps sending the $i$-th marked point to $x_i \in S$ for $i=1,\ldots,g$,
see \cite[Appendix~A]{BL}.

Let $[f:C \to S] \in \Mbar(S,\bx)$.
Thanks to the generality assumption on $(S,L)$, we may and will assume
that $L$ generates the Picard group of $S$. 
The condition $f_* C \in |L|$ thus imposes that $f_*C$ is an integral
cycle, hence that $f$ contracts all irreducible components of $C$ but
one, and restricts to a birational map on the latter component, which
we will call $C_1$.
Now the points $x_1,\ldots,x_g$, being general, impose $g$ general
independent linear conditions on $|L|$, which implies that the curve
$f(C) = f(C_1)$ must have geometric genus at least $g$ by the key fact
mentioned at the beginning of the proof.
Therefore $C_1$ as well  must have geometric genus at least $g$,
and because of the inequality of arithmetic genera
\begin{equation*}
p_a(C_1) \leq p_a(C) = g,
\end{equation*}
this implies that $C_1$ is smooth of genus $g$;
moreover, the stability conditions then imply that $C=C_1$,
hence $f$ is the normalization of the integral genus $g$ curve
$f(C_1)$. 

This already tells us that the space $\Mbar(S,\bx)$ is
$0$-dimensional, and isomorphic as a set to the space of genus $g$
curves in $|L|$ passing through $x_1,\ldots,x_g$.
Since $\Mbar(S,\bx)$ has the expected dimension, the virtual class on
it simply encodes its schematic structure.
It follows that the
number $N^p_g$ is weakly enumerative, \ie it gives the number of genus
$g$ curves passing through $x_1,\ldots,x_g$ counted with
multiplicities.

The fact that these multiplicities all equal $1$ follows from the fact
that all the curves we consider are immersed, as follows.
Let $[f:C \to S] \in \Mbar(S,\bx)$ as above. 
Since $f$ is an immersion, it has normal bundle 
\[
N_f = f^*\omega_S \otimes \omega_C = \omega_C
\]
by \cite[(2.3)]{DS15-10}, 
hence $\h^0(N_f)=g$ and the full moduli space
$\Mbar_{g,0} (S,L)$ is smooth of dimension $g$ at the point $[f]$.
By \cite[Lemma~(2.5)]{DS15-10}, there is a surjective map $e$ from a
neighbourhood of $[f]$ in $\Mbar_{g,0} (S,L)$ onto a neighbourhood of
$f(C)$ in the locally closed subset of $|L|$ parametrizing genus $g$
curves. By generality of the points $x_1,\ldots,x_g$, the latter space
is smooth of dimension $g$ at the point $[f(C)]$.
Therefore $e$ is a local isomorphism at $[f]$, and this implies that
the scheme $\Mbar(S,\bx)$ is reduced at $[f]$, which shows that the
stable map $f$ counts with multiplicity $1$.
\end{proof}

\setcounter{paragraph}{\value{paragraph}+1}
For all integers $g \geq 0$, set
\begin{equation}
\label{eq:defFg}
F_g (q)
:= \sum _{p =g} ^{+\infty} N^p_g \, q^p
\end{equation}
\setcounter{paragraph}{\value{paragraph}-1}
as a formal power series in the variable $q$, where we set $N^0_0$ by
convention so that $F_0$ equals the power series of \eqref{eq:YZ}.
Beware the shift in degree between the definition \eqref{eq:defFg} of
the series $F_g$ and that given in \cite{BL}.
Note that $N^p_g = 0$ whenever $p<g$.

\begin{theorem}[Bryan--Leung]
\label{T:BL}
\setcounter{equation}{1}
The power series $F_g$ is the Fourier expansion of  
\begin{equation}
\label{eq:BL}
\Biggl(
\sum _{n=1} ^{+\infty} n \sigma_1(n)\, q^n
\Biggr)^g\ 
\prod_{m = 1}^{+\infty} \frac 1 {(1-q^m) ^{24}},
\end{equation}
where $\sigma_1(n) := \sum _{d|n} d$ is the sum of all positive integer
divisors of $n$.
\end{theorem}

This formula gives the possibility to explicitly compute as many
numbers $N^p_g$ as we want. Table~\ref{t:BL} (p.~\pageref{t:BL}) gives
sample values for 
small $p$ and $g$. Note that since columns are indexed by
$\delta:=p-g$, the Fourier coefficients of a given $F_g$ are read
along a diagonal; this gives for instance $F_0$ as in \eqref{eq:YZ}, 
\begin{equation*}
F_1(q) = q + 30 q^2 + 480 q^3 + 5460 q^4 +\cdots
\end{equation*}
and so on.

We will discuss the proof of Theorem~\ref{T:BL} in
Section~\ref{s:pf-BL}. 

\begin{table}
\centering
\caption{First values of $N^p_g$ ($\delta=p-g$)}
\label{t:BL}
\rotatebox{90}{
\begin{tabular}{|l||c|c|c|c|c|c|c|c|c|}
\hline
\diagbox {$p$} {$\delta$} & 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 & 9\\
\hline \hline
1 & 24 & &&&&&&& \\
2 & 30 & 324   &&&&&&& \\
3 & 36 & 480   & 3200 &&&&&& \\
4 & 42 & 672   & 5460  & 25650 &&&&& \\
5 & 48 & 900   & 8728  & 49440   & 176256   &&&& \\
6 & 54 & 1164  & 13220 & 88830   & 378420   & 1073720   &&&  \\
7 & 60 & 1464  & 19152 & 150300  & 754992   & 2540160   & 5930496 &&\\
8 & 66 & 1800  & 26740 & 241626  & 1412676  & 5573456   & 15326880   & 30178575    &              \\
9 & 72 & 2172  & 36200 & 371880  & 2499648  & 11436560  & 36693360   & 84602400    & 143184000    \\
10 & 78 & 2580 & 47748 & 551430  & 4213332  & 22116456  & 81993600   & 219548277   & 432841110    \\
11 &    & 3024 & 61600 & 791940  & 6808176  & 40588544  & 172237344  & 531065070   & 1210781880   \\
12 &    &      & 77972 & 1106370 & 10603428 & 71127680  & 342358560  & 1205336715  & 3154067950   \\
13 &    &      &       & 1508976 & 15990912 & 119665872 & 647773200  & 2582847180  & 7698660544   \\
14 &    &      &       &         & 23442804 & 194196632 & 1172896512 & 5255204625  & 17710394230  \\
15 &    &      &       &         &          & 305225984 & 2041899840 & 10205262330 & 38607114200  \\
16 &    &      &       &         &          &           & 3431986848 & 19002853575 & 80149394030  \\
17 &    &      &       &         &          &           &            & 34070137272 & 159184435520 \\
18 &    &      &       &         &          &           &            &             & 303705014550 \\
\hline
\end{tabular}
} % end rotatebox
\end{table}



\paragraph{Modularity}
\label{p:modular}
Formula~\eqref{eq:BL} implies that $qF_g(q)$ is a quasi-modular form
for all $g$.
In the present paragraph I explain what this means; this is also an
occasion to introduce notation for further use (I follow
\cite{serre-arithmetique}).
I will however not try to give a meaningful interpretation of the
(quasi-)modularity of $qF_g(q)$.

\subparagraph{}\smallskip
For every integer $k>1$, define the $k$-th \emph{Eisenstein series} to
be
\begin{equation*}
G_k (z) :=
\sum _{ \substack{
(m,n) \in \Z^2 :\\ (m,n) \neq (0,0)
}}
\frac 1 {(m+nz)^{2k}};
\end{equation*}
it is a modular form of weight $2k$
\cite[Prop.~VII.4]{serre-arithmetique}, which means that it is
holomorphic and $G_k(z) dz^k$ is invariant under the action of
$\mathrm{PSL}_2(\Z)$. Its Fourier expansion at infinity is
\begin{equation*}
G_k(z)=
\frac {2^{2k}} {(2k)!} B_k \pi^{2k}
+2 \frac {(2\pi i)^{2k}} {(2k-1)!}
\sum _{n=1} ^{+ \infty} \sigma_{2k-1} (n) q^n,
\end{equation*}
where $q=e ^{2\pi iz}$,
$\sigma_k(n) = \sum _{d|n} d^k$,
and $B_k$ is the $k$-th Bernoulli number,
defined by the formula
\begin{equation*}
\frac x {e^x-1}
= 1 - \frac x 2
+ \sum _{k=1} ^{+\infty} (-1)^{k+1} B_k \frac {x^{2k}}{(2k)!}
\end{equation*}
\cite[Prop.~VII.8]{serre-arithmetique}.
We set
\begin{align*}
E_k(z) := \frac {(2k)!} {2^{2k} B_k \pi^{2k}} G_k(z)
&= 1 + (-1)^k \frac {4k} {B_k} 
\sum _{n=1} ^{+ \infty} \sigma_{2k-1} (n) q^n \\
&= 1 + (-1)^k \frac {4k} {B_k} 
\sum _{n=1} ^{+ \infty} n ^{2k-1} \frac {q^n} {1-q^n}.
\end{align*}

\subparagraph{}\smallskip
Define
\begin{equation*}
\Delta (z) := \bigl( 60 G_2(z) \bigr)^3 - 27 \bigl(140G_3(z) \bigr) ^2,
\end{equation*}
the discriminant of the cubic polynomial
$4X^3 -60G_2 X - 140G_3$ divided by $16$.
It is a modular form of weight $12$
vanishing at infinity, and it is a theorem of Jacobi 
\cite[Thm.~VII.6]{serre-arithmetique} that
\begin{equation*}
\Delta (z) = (2\pi)^{12} q \prod _{n=1} ^{+\infty} (1-q^n)^{24}.
\end{equation*}

\subparagraph{}\smallskip
In the $k=1$ case, we set
\begin{equation*}
G_1(z) := \sum_{n \in \Z} 
\sum_ {\substack{
m \in \Z: \\ (m,n) \neq (0,0)
}}
\frac 1 {m+nz^2}
\end{equation*}
(note that the order of summation is significant).
It has Fourier expansion at infinity
\begin{equation*}
G_1(z) = \frac {\pi^2} 3
-8\pi^2 \sum _{n=1} ^{+\infty} \sigma_1(n) q^n
\end{equation*}
\cite[\S~VII.4.4]{serre-arithmetique}, and we set
\begin{equation*}
E_1(z) := 
\frac 3 {\pi^2} G_1(z)
= 1 - 24 \sum _{n=1} ^{+\infty} \sigma_1(n) q^n.
\end{equation*}
One has the identity \cite[\S~VII.4.4]{serre-arithmetique}
\begin{equation*}
\frac {d\Delta} \Delta =
2\pi i E_1(z) dz.
\end{equation*}

\subparagraph{}\smallskip
The function $G_1$ is \emph{not} a modular form, but still it does
satisfy a functional equation close to that equivalent to the
invariance of $G_1(z)dz$ under the action of
$\mathrm{PSL}_2(\Z)$ \cite[Prop.~6 p.~19]{123}. For this reason, it is
called a \emph{quasi-modular} form.

One may then define the ring of
quasi-modular forms as the $\C$-algebra generated by $G_1$ and the
algebra of modular forms (see \cite{123} for a more intrinsic
definition).
Since the ring of modular forms is generated by $G_2$ and $G_3$
\cite[Cor.~VII.2]{serre-arithmetique}, the ring of quasi-modular forms
may be concretely described as $\C[G_1,G_2,G_3]$.
The ring of quasi-modular forms is closed under differentiation by the
operator
\begin{equation*}
D:= q \frac d {dq} = \frac 1 {2\pi i}\, \frac d {dz}
\end{equation*}
\cite[Prop.~15 p.~49]{123}.

\subparagraph{Quasi-modularity of $qF_g(q)$}\smallskip
\label{sp:BL-quasimod}
Taking into account the various stunning formul{\ae} above,
\eqref{eq:BL} may be rewritten as
\begin{equation*}
q F_g(q) =
\left( -\frac 1 {24} q\, \frac {dE_1}{dq}
\right) ^g
\left( \frac \Delta {(2\pi)^{12}}
\right) ^{-1},
\end{equation*}
from which it follows that $q F_g(q)$ is a quasi-modular form, with a
simple pole at infinity (\ie at $q=0$) if $g=0$.



\subsection{Proof of the G\"ottsche--Bryan--Leung formula}
\label{s:pf-BL}

This subsection is dedicated to the proof of Theorem~\ref{T:BL}.
As the latter really is about counting actual curves (\ie subvarieties
of the surface), as
Lemma~\ref{l:enum} attests, one may prefer in the first place to avoid
the complications of Gromov--Witten theory to prove it.
Bryan and Leung's proof however goes the orthogonal direction:
it fundamentally
relies on the agile possibilities featured in Gromov--Witten theory,
precisely as a reward to the aforementioned complications.

\paragraph{Degeneration to an elliptic $K3$}
\label{p:degen}
Let $g\geq 0$, $p>0$ be integers. By deformation invariance, we are
free to compute the number $N^p_g$ on our favourite primitively
polarized $K3$ surface $(S,L)$ of genus $p$. We let $S$ be an elliptic
$K3$ surface with a section $E$, and denote by $F$ the class of the
ellitic fibres; the intersection form (or its restriction to the
subspace $\langle E, F \rangle$) is given in the basis $(E,F)$ by the
matrix 
\[
\begin{pmatrix}
-2 & 1 \\ 
1 & 0
\end{pmatrix}.
\]
We set $L:= \O_S(E+pF)$. Then $L^2=2p-2$, and $L$ is a primitive
polarization of genus $p$.
We shall compute the numbers $N^p_g$ on the pair $(S,L)$.


\paragraph{}
\label{p:ell-setup}
The linear system $|E+pF|$ has dimension $p$ and consists solely of
reducible curves $E+F_1+\cdots + F_p$, where the $F_i$'s are in the
class $F$. 
From this it readily follows that if we fix a general set of $g$
points $\by = (y_1,\ldots,y_g)$ on $S$, then the moduli space
\begin{equation*}
\Mbar _{g,\by} (S,E+pF) :=
\Mbar _{g,g} (S,E+pF) \cap \ev_1^* (y_1) \cap \ldots 
\cap \ev_g^* (y_g)
\end{equation*}
of genus $g$ stable maps passing through the points $y_1,\ldots,y_g$
decomposes as the disjoint union
\begin{equation*}
\coprod _{\ba,\bb} \Mbar _{\ba,\bb},
\end{equation*}
where $\ba=(a_1,\ldots,a_{24})$ and $\bb = (b_1,\ldots,b_g)$ range
through $\Z _{\geq 0} ^{24}$ and $\Z _{>0} ^g$ respectively,
subject to the condition that $\sum_i a_i + \sum_j b_j = p$,
and $\Mbar _{\ba,\bb}$ is the moduli space of genus $g$ stable maps
$(f:C \to S,x_1,\ldots,x_g)$ such that $f(x_j)=y_j$ for $j=1,\ldots,g$
and
\begin{equation*}
f_*C = E+\sum _{i=1} ^{24} a_i R_i + \sum _{j=1} ^g b_j F_j,
\end{equation*}
where
$R_1,\ldots,R_{24}$ are the $24$ rational members of the pencil
$|F|$, and $F_j$ being the unique member of $|F|$ containing the point
$y_j$ for all $j=1,\ldots,g$ (see figure below); note that
we may and do assume that all members of $|F|$ are irreducible, and
the $R_i$'s are %pairwise disjoint and 
$1$-nodal.
\begin{center}
%\medskip
\includegraphics[height=3cm]{ellK3.eps}
%\bigskip
\end{center}

\paragraph{Partition function}
\label{p:partition}
For all positive integers $n$, we let $p(n)$ be the \emph {number of
partitions} of $n$, \ie the number of ways to write
$n = \lambda_1 + \cdots + \lambda_k$ with
$\lambda_1 \geq \cdots \geq \lambda_k \geq 1$ ($k$ is not fixed).
The numbers $p(n)$ may be computed using the generating series
\begin{align}
\notag
1+ \sum _{n=1} ^{+ \infty} p(n) \, t^n
&= (1+t^1+t^{1+1}+t^{1+1+1}+\cdots) \times
(1+t^2+t^{2+2}+t^{2+2+2}+\cdots) \\
\notag
& \qquad \qquad \times
(1+t^3+t^{3+3}+t^{3+3+3}+\cdots)\times
\cdots \\
\label{eq:partition}
&= \prod _{n=1} ^{+\infty} \frac 1 {1-t^n}.
\end{align}
See \cite[Chap.~4]{fulton-harris} for much more about this.

\medskip
The following proposition is the key to Formula~\eqref{eq:BL} for an
elliptic $K3$ surface  $(S,L)$ as above.
It yields Formula~\eqref{eq:BL} after a series of
manipulations of generating functions, involving Identity
\eqref{eq:partition}.
I don't reproduce them here, and refer to
\cite[p.~383]{BL} for details.
The rest of this subsection is dedicated to the proof of
the proposition.

\begin{proposition}
\label{pr:BLmain}
The contribution of $\Mbar _{\ba,\bb}$ to $N^p_g$ is
\begin{equation}
\label{eq:BLmain}
\biggl( \prod\nolimits _{i=1} ^{24} p(a_i) \biggr)
\biggl( \prod\nolimits _{j=1} ^g b_j \sigma_1(b_j) \biggr).
\end{equation}
\end{proposition}


\paragraph{Enumeration of elliptic multiple covers}
\label{p:ell-covers-enum}
We first explain the factors $b_j \sigma_1(b_j)$ in
\eqref{eq:BLmain}; they are of a
combinatorial nature.

Let $f:C \to S$ be a member of $\Mbar _{\ba,\bb}$.
It is necessarily shaped as follows: the curve $C$ consists of 
(i) a smooth rational curve mapped isomorphically to the section $E
\subset S$, which we will abusively call $E$ as well, 
(ii) $g$ smooth elliptic curves $G_1,\ldots,G_g$, pairwise disjoint
and each attached at one point to $E$, and
(iii) $24$ trees of smooth rational curves $T_1,\ldots,T_{24}$, pairwise
disjoint, each disjoint from the $G_j$'s and attached to $E$ at one
point.
For all $j=1,\ldots,g$, $f$ maps $G_j$ to the elliptic fibre $F_j$ with
degree $b_j$, and there is a marked point $x_j \in G_j$ mapped to
$y_j$;
for all $i=1,\ldots,24$, one has $f_* T_i = a_i R_i$.
%SEE FIGURE?

For all $j$, we may fix the intersection point with $E$ as the origin
of $G_j$ and $F_j$ respectively, which makes
$\left. f \right|_{G_j}: G_j \to F_j$ a degree $b_j$ homomorphism of
elliptic curves. 
Such homomorphisms are in $1:1$ correspondence with index $b_j$
sublattices of the lattice defining $F_j$ as a complex torus,
and the number of such sublattices is $\sigma_1 (b_j)$
\cite[\S~VII.5.2]{serre-arithmetique}.
In addition, there are $b_j$ possibilities to choose the marked point $x_j$
in the preimage of $y_j$ in $G_j$.

Once the data of the homomorphisms $G_j \to F_j$ and the marked points
$x_j \in G_f$ is fixed, the corresponding sub-moduli space of $\Mbar
_{\ba,\bb}$ decomposes as a product
\begin{equation*}
\prod _{i=1} ^{24} \Mbar _{a_i \be_i,0},
\end{equation*}
where $\be_1=(1,0,\ldots,0), \ldots, \be_{24}=(0,\ldots,0,1) \in \Z ^{24}$.
The moduli space $\Mbar _{\ba,\bb}$ thus consists of 
$\prod _{j=1} ^g b_j \sigma_1(b_j)$ disjoint copies of the space 
$\prod _{i=1} ^{24} \Mbar _{a_i \be_i,0}$, and the rest of the proof
of Proposition~\ref{pr:BLmain}
consists in showing that each of those contributes by 
$\prod _{i=1} ^{24} p(a_i)$ to $N^p_g$.


\paragraph{Description of $\Mbar _{a_i \be_i,0}$}
\label{p:decomp-rat}
Let us start by defining a model stable map 
$h _{a,R}: \bSigma_a \to S$ for
all positive integers $a$ and $1$-nodal rational curves $R \in
\{R_1,\ldots,R_{24}\}$.
%
The curve $\bSigma_a$ is a tree of $2a+2$ smooth rational curves 
$\Sigma_E,\Sigma_{-a},\ldots, \Sigma_0, \ldots \Sigma_{+a}$ as depicted
on the figure below.
\begin{center}
\medskip
\includegraphics[width=\textwidth-.5cm]{lift.eps}
\end{center}

\noindent
The map $h_ {a,R}$ is chosen so that it restricts to an isomorphism
$\Sigma_E \cong E$ 
(hence from now on we will denote $\Sigma_E$ by $E$)
and to $2a+1$ copies $\Sigma_i \to R$ of the
normalization of the $1$-nodal rational curve $R$, in such a way
that it is everywhere a local isomorphism between $\bSigma_a$ and $E
\cup R$. Concretely, the latter requirement is that locally at every
node $\Sigma_i \cap \Sigma_{i+1}$, the map $h_{a,R}$ should send $\Sigma_i$
to one of the two local branches of $R$ at its node and
$\Sigma_{i+1}$ to the other.

There are basically two possible (indifferent) choices. 
We indicate one of them on the above figure by decorating each local
branch at a node of $\Sigma_{-a} \cup \ldots \cup \Sigma_{+a}$ with a
letter $A$ or $B$, with the convention that $A$ and $B$ label the two
local branches of $R$ at its node.


\begin{lemma}
\label{l:lift}
For every $(f: C \to S) \in \Mbar _{a\be_i,0}$, there is a unique
lift of $f$ to a stable map $\tilde f: C \to \bSigma_a$,
meaning that $f = h _{a,R_i} \circ \tilde f$.
\end{lemma}

\begin{proof}
% The proof is algorithmic, and it is best to follow it on an example,
% for instance the one we propose ON FIGURE BLABLA.
% The non-negative integers along irreducible components of $C$ denote
% the degree of the restriction of $f$.
% 
The curve $C$ is necessarily made of a smooth rational component
mapped isomorphically to $E$, which we denote by $E$ as well, and a
tree of smooth rational curves $T$ attached at one point to $E$, as in
\ref{p:ell-covers-enum}. For each irreducible component $C_s$ of $T$,
one has $f_* C_s = k_s R_i$ for some non-negative integer $k_s$.
We determine the lift $\tilde f$ by exploring
the dual graph of $T$ along all possible paths from its root to one of
its leaves, as follows.

There is a unique irreducible component $C_0$ of $T$ intersecting $E$;
we call the corresponding vertex of the dual graph of $T$ the
\emph{root} of the dual graph. 
The \emph{leaves} are those vertices corresponding to irreducible
components of $T$ intersecting only one other irreducible component.
Now the lift $\tilde f$, should it exist, necessarily maps $C_0$ to
$\Sigma_0$, and there is a unique suitable map $C_0 \to \Sigma_0$ 
(possibly contracting $C_0$ to the point $\Sigma_0 \cap E$)
by the universal property of normalization.

Suppose a putative lift $\tilde f$ is determined on an irreducible
component $C_s$ of $T$, and consider an arbitrary component $C_{s+1}$
of $T$ intersecting $C_s$ at one point $z _{s+1}$.
We claim that the behaviour of $\tilde f$ on $C _{s+1}$ is uniquely
determined by the already constructed piece $\tilde f \bigr|
_{C_s}$.
If $C_{s+1}$ is contracted by $f$, this is clear; 
otherwise it is enough, by the universal property of normalization, to
determine which component of $\bSigma_a$ the lift $\tilde f$ should
map $C_{s+1}$ to.
If $\tilde f (z_{s+1})$ is a smooth point of $\bSigma_a$, then $\tilde
f$ has to map $C _{s+1}$ to the same component it maps $C_s$ to;
if not, $\tilde f (z_{s+1})$ is a node $\Sigma _{t_s} \cap \Sigma
_{t_s + \epsilon}$, $\epsilon \in \{ \pm1\}$, and $\tilde f$ has to
map $C _{s+1}$ to $\Sigma _{t_s}$ or $\Sigma _{t_s + \epsilon}$,
depending on which of the local branches $A$ and $B$ of $R_i$ at its
node the local branch of $C_{s+1}$ at $z_{s+1}$ is mapped to by $f$.

This discussion shows that one may algorithmically construct an
$\tilde f$ such that $h _{a,R_i} \circ \tilde f =f$, and that there is a
unique such lift.
(Note that the chain of rational curves $\Sigma _{-a} \cup \ldots \cup
\Sigma_a$ is long enough for the construction to go through without
any trouble: since $f_* C = E+aR_i$,
if at some point during the algorithm we hit
an irreducible component $C_s$ of $C$ that has to be mapped to
$\Sigma_{-a+1}$ or $\Sigma_{a-1}$, 
then the push-forward by $f$ of the sum of all components already
visited by the algorithm fills out the class $aR_i$, hence
all components of $C$ not yet touched by the algorithm are
contracted by $f$, and we don't have to go beyond $\Sigma_{-a+1}$ or
$\Sigma_{a-1}$ in $\bSigma_a$).
\end{proof}

Using Lemma~\ref{l:lift}, one can associate to every stable map
$(f: C \to S) \in \Mbar _{a\be_i,0}$ a combinatorial datum called an
\emph{admissible sequence} of weight $a$: this is a sequence of
$2a+1$ non-negative integers
$\bk = (k_l)_{-a\leq l \leq a}$ with the property
that there exist $m,n \geq 0$
such that
$k_l=0$ for all $l < -m$ and $l > n$,
and $k_l >0$ for all $l=-m,\ldots,n$.
The association goes as follows: let $h_{a,R_i} \circ \tilde f$
be the factorization of $f$, and write
\[
\tilde f _* C = E + \sum _{s=-a} ^a k_s \Sigma_s.
\]
It follows from the construction of $\tilde f$ in the proof of
Lemma~\ref{l:lift} that $(k_{-a},\ldots,k_a)$ is an admissible
sequence of weight $a$.
This gives the following.

\begin{lemma}
\label{l:decompx}
The moduli space $\Mbar _{a\be_i,0}$ decomposes as the disjoint
union 
\begin{equation*}
\Mbar _{a\be_i,0} = 
\coprod _\bk \Mbar _{\bk},
\end{equation*}
where $\bk$ ranges over all weight $a$ admissible sequences, and 
$\Mbar _{\bk}$ is the sub-moduli space of $\Mbar _{a\be_i,0}$
parametrizing those $f$ with associated admissible sequence $\bk$.
\end{lemma}


\paragraph{Identification of the virtual class}
\label{p:id-virt}
It follows from the above that each 
moduli space $\Mbar _{\ba,\bb}$ decomposes
as a disjoint union of various products
$\prod _1 ^{24} \Mbar _{\bk_i}$.
%
% Recall that in \ref{p:ell-covers-enum} we saw the moduli space 
% $\Mbar _{\ba,\bb}$ decomposes in a disjoint union of copies of the product
% $\prod _1 ^{24} \Mbar _{a_i \be_i,0}$
% (each corresponding to a given behaviour over the elliptic fibres
% $F_1,\ldots,F_g$);
% each $\Mbar _{a_i \be_i,0}$ in turn decomposes as a disjoint union of
% moduli spaces $\Mbar _{\bk_i}$ of stable maps with target the curve
% $\bSigma_{a_i}$, with $\bk_i$ an admissible sequence of
% weight $a_i$, as we have described in \ref{p:decomp-rat}.
% Eventually, $\Mbar _{\ba,\bb}$ is thus a disjoint union of various
% products $\prod _1 ^{24} \Mbar _{\bk_i}$.
%
A key point in the proof of Bryan and Leung is the explicit
identification of the restriction to the product $\prod _1 ^{24} \Mbar
_{\bk_i}$ of the (reduced) virtual class giving rise to the invariant
$N^p_g$ 
\cite[\S~5.2]{BL}.
This is by far the most demanding part of their article, and I will not
attempt to give any idea of the proof.

The upshot is that 
(i) the virtual class on $\prod _1 ^{24} \Mbar _{\bk_i}$ is a product
of virtual classes on the various factors, and
(ii) the virtual class on the factor $\Mbar _{\bk_i}$ is computed by
means of a \emph{virtual tangent bundle} on the target curve
$\bSigma _{a_i}$.
This virtual tangent bundle $\stT$ is the vector bundle on
$\bSigma_{a_i}$ defined by the conditions that it is isomorphic to 
$h _{a_i,R_i} ^* T_S$ on $\Sigma_{-a} \cup \ldots \cup \Sigma_a$
and to $T_E \oplus \O_E(-1)$ on $E$.

Note that $h _{a_i,R_i} ^* T_S$ restricts to $T_E \oplus \O_E(-2)$ on
$E$; the correction made to define $\stT$ corresponds to the fact that
we want to kill the obstruction space $H^1(C,N_f)$ as we know the
actual obstruction space is trivial although $H^1(C,N_f)$ is not, see
\ref{p:redGW}.

\paragraph{Planar model}
\label{p:planar}
Let $a$ be a non-negative integer.
Thanks to the result discussed in \ref{p:id-virt},
it is possible to construct a
model for $\bSigma_a$ embedded in a familiar surface $P$, such that
the actual deformation theory of $\bSigma_a$ in $P$ is isomorphic
to the reduced virtual theory leading to the
invariants $N^p_g$. This will eventually let us compute the
contribution of the $\Mbar _{\bk_i}$'s (hence also of the $\prod _1
^{24} \Mbar _{\bk_i}$'s) to the invariant $N^p_g$.

Let  $p,p_{-1},p_1$ be three distinct points lying on a line in
the projective plane $\P^2$. 
Let $P_1 \to \P^2$ be the blow-up at these three points, and call $E$
the exceptional divisor over $p$, $\Sigma_0$ the proper transform of
the line through $p,p_{-1},p_1$, and $\Sigma_{-1}, \Sigma_1$ the
exceptional divisors over $p_{-1},p_1$ respectively.
Next, recursively for all $s=1,\ldots,a$, we perform the blow-up
$P_{s+1} \to P_s$ at two general points of $\Sigma_{-s}$ and
$\Sigma_s$ respectively, and let $\Sigma_{-s-1}$ and $\Sigma_{s+1}$ be
the two corresponding exceptional divisors;
we call $E,\Sigma_{-s},\dots,\Sigma_s$ the proper
transforms in $P_{s+1}$ of the curves with the same name in $P_s$.

The curve $\Sigma_{-a} \cup \ldots \cup \Sigma_0 \cup \ldots \cup
\Sigma_a$ in $P_{a+1}$
(note that this excludes the last two exceptional curves
$\Sigma_{-a-1}$ and $\Sigma _{a+1}$) is isomorphic as an abstract
curve to $\bSigma_a$. Moreover, the tangent bundle of $P_{a+1}$
restricts to $\O _{\P^1} (2) \oplus \O _{\P^1} (-1)$ on $E$, and to 
$\O _{\P^1} (2) \oplus \O _{\P^1} (-2)$ on
$\Sigma_{-a},\ldots,\Sigma_a$;
it is therefore isomorphic to the virtual tangent bundle $\stT$
introduced in \ref{p:id-virt}.
Then, Bryan--Leung prove the following.

\begin{lemma}
\label{l:GWasP2}
For all admissible sequences $\bk=(k_{-a},\ldots,k_0,\ldots,k_a)$, the
``local'' contribution $\int _{[\Mbar _\bk] ^{\rm vir}} 1$
of $\Mbar _\bk$ to the invariant $N^p_g$ equals the
ordinary genus $0$ Gromov--Witten integral
$\int _{[\Mbar_0 (P_{a+1},\beta)] ^{\rm vir}} 1$
for the class
$\beta = E + \sum _{-a} ^a k_s \Sigma_s$.
\end{lemma}


The lemma follows from \ref{p:id-virt} and the isomorphism between the
restriction of $T _{P_{a+1}}$ and $\stT$ to $\bSigma_a$,
provided the two moduli
spaces $\Mbar _\bk$ and the ordinary
$\Mbar_0(P_{a+1}, E + \sum _{-a} ^a k_s \Sigma_s)$ are isomorphic as 
sets.
Bryan and Leung are able to prove this by elementary arguments using a
more elaborate set-up: they start with a linear $\C^*$ action
(not $(\C^*)^2$)
on $\P^2$ leaving the line $\langle p,p_{-1},p_1 \rangle$ and a point
$q$ fixed, and this $\C^*$ action survives in $P_{a+1}$. See
\cite[Lemma~5.7]{BL} for the proof.

Finally, by deformation invariance of Gromov--Witten invariants, we
may transport the computation on the projective plane blown-up at
$2a+3$ general points. This gives the following.

\begin{lemma}
\label{l:GWasP2fin}
Let $\tilde \P^2$ be the blow-up of $\P^2$ at a general set of $2a+3$
points, with exceptional divisors
$E,E_{-a-1},\ldots,E_{-1},E_1,\ldots,E_{a+1}$ 
(all $(-1)$-curves of course). We call $H$ the pull-back of the line
class. 
Then for all admissible sequences $\bk=(k_{-a},\ldots,k_0,\ldots,k_a)$, the
``local'' contribution $\int _{[\Mbar _\bk] ^{\rm vir}} 1$
of $\Mbar _\bk$ to the invariant $N^p_g$ equals the
ordinary genus $0$ Gromov--Witten integral 
$
\int _{[\Mbar_0 (\tilde\P^2,\beta _\bk)] ^{\rm vir}} 1
$
for the class
\begin{align*}
\beta _\bk &=
E+ \sum _{s=1} ^{a} k_{-s} (E_{-s}-E_{-s-1})
+ k_0 (H-E-E_1 -E_{-1})
+ \sum _{s=1} ^{a} k_{s} (E_{s}-E_{s+1}) \\
&=
k_0 H -(k_0-1)E
- \sum _{s=1} ^a (k_{s-1}-k_s) E_s -k_a E_{a+1}
- \sum _{s=1} ^a (k_{-s+1}-k_{-s}) E_{-s} -k_{-a} E_{-a-1}.
\end{align*}
\end{lemma}

\noindent
Note that 
\begin{equation*}
(k_0-1)
+ \sum _{s=1} ^a (k_{s-1}-k_s) +k_a
+ \sum _{s=1} ^a (k_{-s+1}-k_{-s}) +k_{-a} 
= 3k_0-1,
\end{equation*}
so the virtual class $[\Mbar_0 (\tilde \P^2,\beta _\bk)] ^{\rm vir}$
has dimension $0$, see \ref{p:P2comput} below.


\paragraph{The computation on the blown-up plane}
\label{p:P2comput}
The Gromov--Witten invariants gotten in Lemma~\ref{l:GWasP2fin} are
computable in practice thanks to the analysis of genus $0$
Gromov--Witten invariants of blow-ups of $\P^2$ carried out by
G\"ottsche and Pandharipande \cite{goettsche-pandharipande}.

Let $n$ be a non-negative integer, $d,\alpha_1,\ldots,\alpha_n$
integers. We call $N(d;\alpha_1,\ldots,\alpha_n)$ the genus $0$
Gromov--Witten invariant for $\tilde \P^2$ and the class
$dH-\sum_i \alpha_i E_i$ (mind the minus sign, introduced for obvious
geometric reasons), where $\tilde \P^2$ is the projective plane
blown-up at a general set of $n$ points, $H$ the pull-back of the line
class, and $E_1, \ldots, E_n$ the exceptional $(-1)$-curves.
The corresponding moduli space of stable maps has virtual dimension
$3d-1-\sum_i \alpha_i$; if this is positive, then we impose in
addition the
appropriate number of point constraints, and if this is negative, then
we set the invariant to $0$.

These invariants enjoy the following properties
(see \cite{goettsche-pandharipande}):
{\setlength{\parindent}{0mm}
\begin{asparaenum}[(i)]
\item $N(1)=1$;
\item
\label{prop:triv}
 $N(d;\alpha_1,\ldots,\alpha_{n-1},1)
= N(d;\alpha_1,\ldots,\alpha_{n-1},0)
= N(d;\alpha_1,\ldots,\alpha_{n-1})$;
\item $N(d;\alpha_1,\ldots,\alpha_n)
= N(d;\alpha_{\sigma(1)},\ldots,\alpha_{\sigma(n)})$
for any permutation $\sigma \in \mathfrak{S}_n$;
\item 
\label{propP2:vanish}
$N(d;\alpha_1,\ldots,\alpha_n) =0$ if there is an index $i$ for
which $\alpha_i <0$,
unless $dH-\sum_i \alpha_i E_i = E_{i_0}$ for some $i_0$ in which case
the invariant is $1$;
\item 
\label{prop:Cr}
The invariant
$N(d;\alpha_1,\alpha_2,\alpha_3,\alpha_4,\ldots,\alpha_n)$
is invariant under the isomorphism given by the quadratic Cremona
transformation corresponding to the linear system
$|2H-E_1-E_2-E_3|$, \ie
\begin{multline*}
N(d;\alpha_1,\alpha_2,\alpha_3,\alpha_4,\ldots,\alpha_n) = \\
N(2d-\alpha_1-\alpha_2-\alpha_3,
d-\alpha_2-\alpha_3,
d-\alpha_1-\alpha_3,
d-\alpha_1-\alpha_2,
\alpha_4,\ldots,\alpha_n).
\end{multline*}
\end{asparaenum}
}

We need the following definition to state the result.
An admissible sequence $(k_{-a},\ldots,k_0,\ldots,k_a)$ is
\emph{$1$-pyramidal}\footnote
{this is called \emph{$1$-admissible} in \cite{BL}.}
if
\[
k_s -1 \leq k_{s+1} \leq k_s
\qquad \text{and} \qquad
k_{-s} -1 \leq k_{-s-1} \leq k_{-s}
\]
for all $s=0,\ldots, a-1$.

\begin{lemma}
\label{l:GWonP2}
Let $\bk=(k_{-a},\ldots,k_0,\ldots,k_a)$ be an admissible sequence of
weight $a$.
Then the genus $0$ Gromov--Witten invariant
\begin{multline*}
  N(\bk):=
  \int _{[\Mbar_0 (\tilde\P^2,\beta _\bk)] ^{\rm vir}} 1
\\  =
N(k_0;\, k_0-1,\,
k_{-a},\,k_{-a+1}-k_{-a},\,\ldots,\,k_0-k_{-1},\,
k_0-k_1,\,\ldots,\,k_{a-1}-k_a,\,k_a)
\end{multline*}
equals $1$ if $\bk$ is $1$-pyramidal, and $0$ otherwise.
\end{lemma}



\begin{proof}
We first show that $N(\bk)=0$ if $\bk$ is not $1$-pyramidal. Since
$k_0 >0$ by definition of an admissible sequence, it follows from 
Property~\eqref{propP2:vanish} above that $N(\bk) \neq 0$ implies
\setcounter{equation}{\value{subparagraph}}
\begin{equation}
\label{GWonP2:ineq1}
k_{-s} \leq k_{-s+1}
\qquad \text{and} \qquad
k_{s-1} \geq k_s
\end{equation}
for all $s =1,\ldots,a$.
Next, we apply
for all $s=2,\ldots,a-1$
the Cremona transformation defined by
$|2H-E-E_1-E_{s+1}|$
and get
\begin{equation*}
N(\bk)=
N(1+k_1+k_{s+1}-k_s; \,
\underbrace{k_1-k_s+k_{s+1}}_{E}, \,\ldots,\,
\underbrace{1-k_s+k_{s+1}}_{E_1}, \,\ldots,\,
\underbrace{1-k_0+k_1}_{E_{s+1}}, \,
\ldots\,)
\end{equation*}
by Property~\eqref{prop:Cr} above.
If $N(\bk) \neq 0$, we have $k_s \leq k_1$ by \eqref{GWonP2:ineq1},
hence $1+k_1+k_{s+1}-k_s >0$, and Property~\eqref{propP2:vanish} then
implies that $k_1 \geq k_0-1$ and $k_{s+1} \geq k_s-1$.  An analogous
move shows that $k_{-s-1} \geq k_{-s} -1$ for all $s=0,\ldots,a-1$ if $N(\bk)
\neq 0$. Thus, the non-vanishing of $N(\bk)$
implies that $\bk$ is $1$-pyramidal.

Conversely, assume that $\bk$ is $1$-pyramidal of weight
$a$. Then $k_a = k_{-a} =0$ (otherwise the weight exceeds $a$; we have
somehow already made this observation in the course of the proof of
Lemma~\ref{l:lift}), and all coefficients $k_s-k_{s-1}$ and
$k_{-s}-k_{-s+1}$ for $s=1,\ldots,a$, equal $0$ or $1$. It thus
follows from Property~\eqref{prop:triv} that
$N(\bk) = N(k_0; k_0-1)$, which is readily seen to equal $1$:
the moduli space of genus $0$ stable maps 
$\Mbar_0 \bigl( \tilde\P^2,k_0H-(k_0-1)E \bigr)$ has only one enumeratively
meaningful irreducible component, isomorphic to the family of
degree $k_0$ plane curves with multiplicity $k_0-1$ at a fixed point
$x_E \in \P^2$, and this is a linear system.
\end{proof}


\noindent
The proof of Theorem~\ref{T:BL} will be complete once we show the
following combinatorial result.

\begin{lemma}
\label{l:combine}
The number of $1$-pyramidal admissible sequences
$(k_{-a},\ldots,k_0,\ldots,k_a)$
of weight $a$ equals the partition number $p(a)$
(\cf \ref{p:partition}).
\end{lemma}


Indeed, together with  Lemmata \ref{l:decompx}, \ref{l:GWasP2fin}
and \ref{l:GWonP2}, 
this shows that the ``local'' contribution of $\Mbar _{a_i \be_i,0}$
equals $p(a_i)$, hence the contribution of each copy of the product
$\prod_1 ^{24} \Mbar _{a_i \be_i,0}$ equals
$\prod_1 ^{24} p(a_i)$;
this proves Proposition~\ref{pr:BLmain},
thanks to the enumeration of elliptic multiple covers performed in
\ref{p:ell-covers-enum}.
Finally, as already mentioned,
Proposition \ref{pr:BLmain} implies Theorem~\ref{T:BL}.


\begin{proof}[Proof of Lemma~\ref{l:combine}]
Partitions of an integer $a$ are in bijective correspondence with
Young diagrams of size $a$ \cite[Chap.~4]{fulton-harris}.
We shall exhibit a bijective correspondence between Young diagrams of
size $a$ and $1$-pyramidal admissible sequences 
$(k_{-a},\ldots,k_0,\ldots,k_a)$
of weight $a$.
We see Young diagrams as embedded in the
upper-right quadrant of a Cartesian plane, leaning on both the $x$
and $y$ axes, and with blocks squares of size $1$. 
Given such a Young diagram, we let $k_s$ be the number of blocks on the
line $y-x=s$ for all $s=-a,\ldots,0,\ldots,a$:
see the figure below for an example of this procedure.
\begin{center}
\includegraphics{pyramid.eps}
\end{center}
We leave it to the reader to check that $(k_{-a},\ldots,k_a)$ is
indeed admissible, $1$-pyramidal, of weight $a$, and that this
correspondence establishes the announced bijection.
\end{proof}


\section{BPS state counts}
\label{S:BPS}

In this Section, I discuss why and how curve counting in non-primitive
classes imply the use of multiple covers formul{\ae}.
This features the generalization of the Yau--Zaslow formula of
Theorem~\ref{T:YZ} to non-primitive classes.

\subsection{Rational curves on the quintic threefold}
\label{s:quintic}

To describe the picture in its simplest form, 
let us first discuss a question that lies slightly outside the scope
of these notes,
namely that of counting rational curves on a general quintic
hypersurface $V$ of $\P^4$.

\paragraph{}
\label{p:vdimCY}
The Clemens conjecture (see \ref{c:clemens} below) predicts that
there are
finitely many such curves of any given degree $d$, in keeping
with the virtual dimension
\begin{equation}
\label{eq:vdim}
\vdim \overline{M}_g(V,\beta)
= (\dim V - 3)(g-1)-K_V \cdot \beta
\end{equation}
being $0$ for any homology class on a Calabi--Yau threefold $V$.
This suggests that the number
\[
N^V_{d} := \int _{[\overline{M}_0(V,d\ell)]^{\rm vir}}
1
\]
(where $\ell$ denotes the homology class of a line) may give
the actual number of rational curves of degree $d$ in $V$.
This would be particularly appealing, since the numbers $N^V_d$ may in
theory be rigorously computed using the predictions of mirror
symmetry; this has been done in practice for small values of $d$,
see \cite{cox-katz} for a thorough discussion.

A first objection against such an ideal correspondence is that
there may 
be rational curves with non-trivial infinitesimal deformations, but
the Clemens conjecture also predicts that this does not happen.

\paragraph{Multiple cover formula}
\label{p:mult-cov}
An actual issue preventing $N_d^V$ from directly reflecting the number of
degree $d$ rational curves on $V$ is the existence of
components of $\overline{M}_0(V,d\ell)$ having dimension larger than
expected (\ie positive dimension).
Suppose there is a smooth degree $d_0=d/k$ rational curve $\Gamma
\subset V$ for some integer $k>1$,
and let $f_0:\P^1 \to V$ be the stable map induced by the 
normalization of $\Gamma$.
Then, for all degree $k$ covers $\phi_k:\P^1\to \P^1$, the composed
map
$f_0\circ \phi_k$ is a member of $\overline{M}_0(V,d\ell)$, and
the locus in $\overline{M}_0(V,d\ell)$ corresponding to such
composed maps over $\Gamma$
is an irreducible variety $M_{k}(\Gamma)$ of dimension $2k-2$.
% \begin{equation}
% \label{eq:mult-cov}
% \P^1 \xrightarrow{k:1} \P^1 \xrightarrow{f} V
% \end{equation}
% \setcounter{subparagraph}{\value{equation}}


% \medskip
% \subparagraph{}
% \setcounter{equation}{\value{subparagraph}}
% {\it
The Aspinwall--Morrison formula asserts that the
corresponding irreducible component $\overline{M}_{k}(\Gamma)$ of
$\overline{M}_0(V,d\ell)$ contributes by $\frac 1 {k^3}$ to the
integral $N^V_{d}$.
This has been mathematically proved by Kontsevich and Manin, and
Voisin,
see
\cite[\S~5.6]{claire-miroir} and \cite[Thm.~7.4.4]{cox-katz}.

To make this plausible it is
convenient to consider, instead of the integrals $N^V_d$,
their close cousins
\[
\langle I^{V}_{0,3,d\ell} \rangle (\omega_1, \omega_2, \omega_3)
:= \int _{[\overline{M}_{0,3}(V,d\ell)]^{\rm vir}}
\ev_1^* (\omega_1) \wedge
\ev_2^* (\omega_2) \wedge
\ev_3^* (\omega_3), 
\]
where $\overline{M}_{0,3}(V,d\ell)$ is the space of genus $0$ stable
maps with $3$ marked points, and the $\omega_i$ are Kähler
forms on $V$.
The moduli space $\overline{M}_{0,3}(V,d\ell)$ has the advantage
over $\overline{M}_0(V,d\ell)$
that it identifies with the Hilbert scheme $\Hom(\P^1,V)$,
locally at those stable maps having source $\P^1$.
Now, it follows from the divisorial axiom of Gromov--Witten theory that
\[
\langle I^{V}_{0,3,d\ell} \rangle (\omega_1, \omega_2, \omega_3)
= \int _{d\ell} \omega_1
\times  \int _{d\ell} \omega_2
\times  \int _{d\ell} \omega_3
\times N^V_d.
\]
On the other hand, each physical degree $d$ rational curve $C \subset V$
contributes via its normalization $f: \P^1 \to V$ by
\[
\int _{\P^1} f^* \omega_1
\times \int _{\P^1} f^* \omega_2
\times \int _{\P^1} f^* \omega_3
\]
to the integral
$\langle I^{V}_{0,3,d\ell} \rangle (\omega_1, \omega_2, \omega_3)$,
hence by
\[
  \frac
  {\bigl(\int _{\P^1} f^* \omega_1\bigr)
    \bigl(\int _{\P^1} f^* \omega_2\bigr)
    \bigl(\int _{\P^1} f^* \omega_3\bigr)
  }
  {\bigl(\int _{d\ell} \omega_1\bigr)
    \bigl(\int _{d\ell} \omega_2\bigr)
    \bigl(\int _{d\ell} \omega_3\bigr)
  }
\]
to the invariant $N_d^V$.
The contribution of $\Gamma$ to $N_{d_0}^V$ may be expressed in the
same way.

Now, suppose we knew what the compactification $\overline{M}_k(\Gamma)$ of
$M_k(\Gamma)$ in $\overline{M}_{0,3}(V,d\ell)$ looks like, and we had a
vector bundle $E$ over it having fibre over $(f_0\circ\phi_k) \in
M_k(\Gamma)$  
the obstruction space $H^1(\P^1,(f_0\circ\phi_k)^*\, T_V)$.
Then we could compute the contribution of $\overline{M}_k(\Gamma)$
to $\langle I^{V}_{0,3,d\ell} \rangle (\omega_1, \omega_2, \omega_3)$
by the excess formula
\begin{equation}
\label{eq:AM-excess}
\int_ {\overline{M}_k(\Gamma)} c_{2k-2}(E) \wedge 
\ev_1^* (\omega_1) \wedge
\ev_2^* (\omega_2) \wedge
\ev_3^* (\omega_3).
\end{equation}
The computation of 
\cite[p.~115--116]{claire-miroir}
shows that a heuristic model for $\overline{M} _k(\Gamma)$ leads to the
following expression for this excess contribution:
\begin{equation*}
\int _{\P^1} f_0^* \omega_1
\times \int _{\P^1} f_0^* \omega_2
\times \int _{\P^1} f_0^* \omega_3.
\end{equation*}
The upshot is that the direct contribution of $\Gamma$ to $N_{d_0}^V$
and its contribution via $\overline{M} _k(\Gamma)$
to $N_d^V$ (in this heuristic model) are, respectively,
\[
  \frac
  {\bigl(\int _{\P^1} f_0^* \omega_1\bigr)
    \bigl(\int _{\P^1} f_0^* \omega_2\bigr)
    \bigl(\int _{\P^1} f_0^* \omega_3\bigr)
  }
  {\bigl(\int _{d_0\ell} \omega_1\bigr)
    \bigl(\int _{d_0\ell} \omega_2\bigr)
    \bigl(\int _{d_0\ell} \omega_3\bigr)
  }
  \et
  \frac
  {\bigl(\int _{\P^1} f_0^* \omega_1\bigr)
    \bigl(\int _{\P^1} f_0^* \omega_2\bigr)
    \bigl(\int _{\P^1} f_0^* \omega_3\bigr)
  }
  {\bigl(\int _{d\ell} \omega_1\bigr)
    \bigl(\int _{d\ell} \omega_2\bigr)
    \bigl(\int _{d\ell} \omega_3\bigr)
  }.
\]
The latter is $\frac 1 {k^3}$ times the former, since
$\int _{d\ell} \omega_i = k \int _{d_0\ell} \omega_i$ for all
$i=1,2,3$.


\paragraph{Instanton numbers}
\label{p:instanton}
The idea is to define new invariants $n^V_d$ from the Gromov--Witten
integrals $N^V_d$ that better reflect the enumerative geometry of the
Calabi--Yau threefold $V$, taking into account the multiple cover
phenomenon described in paragraph \ref{p:mult-cov} above.
The relations that these numbers should satisfy are
\begin{equation}
\label{eq:instantons}
N^V_d = \sum _{k | d} \tfrac 1 {k^3} \, n^V _{d/k}
\end{equation}
for all positive integers $d$, where the sum runs over all positive
integral divisors of $d$. They form an invertible triangular set of
relations, and each number $n^V_d$ is therefore uniquely
determined by the invariants $N^V_{d'}$ for all positive divisors $d'$
of $d$.
These numbers $n_d^V$ are traditionally called
\emph{instanton numbers}. This name obviously bears some physical
meaning, but let me not try to discuss it.


\paragraph{Reducible covers of singular curves}
\label{p:phenom-pandha}
There is yet another phenomenon, first observed by Pandharipande, that
prevents the instanton numbers $n^V_d$ defined in \ref{p:instanton}
above from being the actual numbers of integral degree $d$ rational curves
on $V$.
It comes from the existence of singular integral rational curves.

To describe the simplest instance of this phenomenon,
assume there is a degree $d$ integral rational curve $C \subset V$
with an ordinary 
double point $x$. Let $f: \P^1 \to V$ be the normalization of $C$, and
denote by $x_1$ and $x_2$ the two points in the preimage of $x$ in
the normalization,
Now, consider the map
\begin{equation*}
f_x: \P^1 \cup _{x_1,x_2} \P^1 \to V,
\end{equation*}
obtained by glueing tranversaly two copies
of the normalization of $C$, in such a way that $x_1$ in the first
copy is identified with $x_2$ in the second copy.
It is a stable
map of genus $0$ realizing the homology class $2[C]$ on $V$, hence it
contributes to the Gromov--Witten invariant $N^V_{2d}$.
This contribution is by $1$ if $C$ is infinitesimally
rigid, \cf \cite[\S~9.2.3]{cox-katz}. It follows that a
$\delta$-nodal rational curve of degree $d$ (\ie a curve with exactly
$\delta$ ordinary double points as singularities) contributes 
in the above described fashion by $\delta$ to the Gromov--Witten
integral $N^V_{2d}$.


\medskip
The Clemens conjecture below predicts that the
complications don't go beyond this in the case of a general quintic
threefold. 
Note in particular that part (iii) of the conjecture implies that the
numbers $N^V_d$ (or $n^V_d$) count \emph{irreducible} physical
rational curves $C \subset V$, since by definition the source of a
stable map is connected.
\begin{conjecture}[Clemens]
\label{c:clemens}
Let $V \subset \P^4$ be a general quintic hypersurface.\\
(i) For each integer $d \geq 1$, there are only finitely many
irreducible rational curves $C \subset V$ of degree $d$.\\
(ii) For every integral rational curve $C \subset V$ with
normalisation $f: \P^1 \to V$, the normal bundle $N_f$ of the map $f$
is isomorphic to $\O _{\P^1} (-1) \oplus \O _{\P^1} (-1)$ (\ie $C$ is
infinitesimally rigid).\\
(iii) \emph{All} the integral rational curves on $V$ (of any degree)
are pairwise disjoint.
\end{conjecture}

It is completely proved in degree $\leq 11$
(\cf \cite{ethan11,dalmeida} for the latest steps), and part (i) is
known in degree $12$ \cite{ballico-fontanari}.

%\medskip
We end this prologue about quintic threefolds by an explicit example
displaying all these phenomena together.

\paragraph{Rational curves of degree $10$ on a quintic threefold}
(\cf \cite[\S~9.2.3]{cox-katz} for a thorough analysis).
First note that, by definition of the instanton numbers, the
Gromov--Witten integral $N^V_{10}$ decomposes as
\begin{equation*}
N_{10} = 
\frac 1 {10^3} n_1
+ \frac 1 {5^3} n_2
+ \frac 1 {2^3} n_5
+ n_{10}
\end{equation*}
(we have now dropped the superscript $V$ to lighten notations),
and one has
\begin{align*}
n_1 &= 2,875 \\
n_2 &= 609,250 \\
n_5 &= 229,305,888,887,625 \\
n_{10} &= 704,288,164,978,454,686,113,488,249,750,
\end{align*}
\cf \cite{CdGP}.
While $n_1$ and $n_2$ are simply the numbers of lines and conics
on a general quintic threefold, $n_5$ counts two kinds of
rational curves of degree $5$. 
Indeed, the planes in $\P^4$ are parametrized by a $6$-dimensional
Grassmannian, and for a general quintic $V \subset \P^4$, finitely many
of them are $6$-tangent to $V$; the corresponding plane sections of
$V$ are $6$-nodal plane quintic curves, and in particular they are
rational curves. Vainsencher \cite{vainsencher-10} has been able to
compute their number
\begin{equation*}
n_5' = 17,601,000,
\end{equation*}
see \cite[Paragraph \tref{p:solids2:6nod-5ics}]{14.th-vainsencher}.
Each such curve contributes to $n_5$ (or $N_5$) by $1$
\cite[Lemma~9.2.4]{cox-katz}, and
\begin{equation*}
n_5'' := n_5 - n_5'
\end{equation*}
is indeed the number of \emph{smooth} rational curves of degree $5$ on
$V$. 

Whereas $n_5$ still is the number of rational curves of degree
$5$ on $V$, this is no longer true for $n_{10}$ as the discussion in
\ref{p:phenom-pandha} indicates. The actual number of degree $10$
integral rational curves on $V$ is
\begin{equation*}
n_{10}^\circ := n_{10} - 6 n_5'
\end{equation*}
\cite[Thm.~9.2.6]{cox-katz}\footnote
{there is a misprint there: $6\frac 1 8$ should be replaced by
$6+\frac 1 8$.}.



\subsection{Degree $8$ rational curves on a sextic double plane}
\label{s:gathmann}

In this subsection we give the enumerative interpretation due to
Gathmann \cite{gathmann-conics} of the reduced Gromov--Witten
invariant
\[
N^2_{0,2} :=
\int _{[ \overline{M}_0(S,2L)]^{\rm red}} 1
\]
of a general primitively polarized $K3$ surface $(S,L)$ of genus $2$
(\ie $S$ is a double covering of the plane $\pi:S \to
\P^2$ branched over a general sextic curve $B$, and $L$ is the
pull-back of the line class).
Note that the polarization $2L$ has genus $5$, as
$(2L)^2=8$.

\paragraph{}
\label{p:gath-enum}
{\renewcommand{\thesubparagraph}{(\roman{subparagraph})}
The analysis carried out in Section~\ref{s:quintic} indicates that
the integral $N^2_{0,2}$ is a sum of contributions corresponding to
the following types of curves.
\subparagraph{}
\label{sp:gath-5tg}
 $5$-nodal integral curves in $|2L|$; these are the preimages of
the conics in $\P^2$ tangent to the branch sextic $B$ at $5$ distinct
points. There are $70,956$ of those, as Gathmann was able to compute
using his theory of relative Gromov--Witten invariants for
hypersurfaces.
\subparagraph{}
\label{sp:gath-red1}
Reducible rational curves made of two distinct rational curves in
$|L|$: let $C_1,C_2 \in |L|$ be two rational curves (each of these is the
pull-back of a line bitangent to $B$);
they intersect transversely in two points $x,x'$ where both of them are
smooth, if $(S,L)$ is general; then,
the partial normalization of $C_1+C_2$ at the four nodes of $C_1$ and
$C_2$ and one node among $x$ and $x'$ gives a stable map with source a
chain of two smooth rational curves, mapping birationally onto
the physical curve $C_1 + C_2 \in |2L|$.
% There are correspondingly two distinct stable maps
% \[
% f: \P^1 \cup_{f_1^{-1}(x),f_2^{-1}(x)} \P^1 \to S
% \quad \text{and} \quad
% f': \P^1 \cup_{f_1^{-1}(x'),f_2^{-1}(x')} \P^1 \to S
% \]
% with source the union of two $\P^1$'s meeting transversely at one
% point, which realize the physical curve $C_1 + C_2 \in |2L|$.

These two stable maps contribute each by $1$ to $N^2_{0,2}$, so
in the upshot each of the
$\binom {324} 2$ pairs of distinct rational curves in $|L|$
contributes by $2$ in this way, thus giving a total contribution of
$104,652$ to $N^2_{0,2}$
(recall that there are $324$ bitangent lines to $B$, as can be
classicaly computed, or extracted from Theorem~\ref{T:YZ}).

\subparagraph{}
\label{sp:gath-red2}
Reducible double coverings of one rational curve in $|L|$, as in 
\ref{p:phenom-pandha}. Since all rational curves in $|L|$ are
$2$-nodal, all $324$ of them give $2$ stable maps with reducible
source, contributing by $1$ each to $N^2_{0,2}$, for a total
contribution of $648$.

\subparagraph{} 
Irreducible double covers of one rational curve in $|L|$, as in
\ref{p:mult-cov}.
Gathmann \cite[Lemma~4.1]{gathmann-conics} proved that
each of the $324$ corresponding positive-dimensional irreducible
components of $\overline{M}_0(S,2L)$ gives a contribution
by $\frac 1 8$ to $N^2_{0,2}$, similar
to the prediction of the Aspinwall--Morrison formula, although
we are in a significantly different situation
(we are not on a Calabi--Yau threefold, and the rational curves we are
considering double covers of are singular, for instance).

%end of redef of \thesubparagraph
}


\paragraph{Remark}
An important difference with the case of the quintic threefold,
although rather innocent-looking, is that in the present situation
integral rational curves do intersect each other, contrary to the
prediction of part (iii) of Clemens' Conjecture.
In the above discussion~\ref{p:gath-enum},
this amounts to case~\ref{sp:gath-red1} needing
to be added with respect to the discussion for quintic
threefolds, which is still manageable.
% In the case
% specifically under consideration in this subsection, 
% which has 
When looking at linear systems $|mL|$ with $m \geq 3$ however,
this soon gets much more complicated, see \ref{p:still-not-enum}.



\paragraph{}
\label{p:gath-interp}
From the enumeration of \ref{p:gath-enum}, one may deduce the value of
$N^2_{0,2}$, which was not known before. 
But the striking observation of \cite{gathmann-conics} is that the sum
of the contributions \ref{sp:gath-5tg}--\ref{sp:gath-red2} above, which
would be the instanton number $n^2_{0,2}$ in the language of
\ref{p:instanton}, actually equals 
\[
N^5_{0,1} := N^5_{0} = 176,256,
\]
the number of degree $8$ rational curves in a primitively polarized
$K3$ surface of genus $5$, computed by formula~\eqref{eq:YZ}.
This suggests the amazing possibility that the number of rational
curves in a linear system $|L|$ on a $K3$ surface is independent of
the divisibility of the line bundle $L$.
We will come back to this in
detail in Section~\ref{s:YZ-gen} below.


\subsection{Elliptic curves in a $2$-divisible class on a 
$K3$ surface}
\label{s:lee-leung}

Here, I report on the computation by Lee and Leung
\cite{lee-leung-elliptic} of the reduced Gromov--Witten invariant
\[
N^p_{1,2} :=
\int _{[ \overline{M}_{1,1}(S,2L)]^{\rm red}} \ev_1^* (\mathrm{pt})
\]
of a general primitively polarized $K3$ surface $(S,L)$ of genus $p$,
which ``counts'' genus $1$ curves in $|2L|$ passing through $1$
general point on $S$.
 Using a suitable version of topological recursion, they prove the
following formula.

\begin{theorem}
\label{T:lee-leung}
{\normalfont \! \cite{lee-leung-elliptic}}
One has
\[
N^p_{1,2} = N^{4p-3}_{1,1} + 2 N^p_{1,1}.
\]
\end{theorem}

\noindent
The numbers $N^q_{1,1}:= N^q_1$ are those giving the number of
elliptic curves through a general point in the primitive class of a
 $K3$ surface of genus $q$, as in formula \ref{T:BL}.
Note that $p':=4p-3$ is the genus of the polarization $2L$, \ie
$(2L)^2=2p'-2$.

\paragraph{}
Lee and Leung propose the following interpretation of their
formula~\ref{T:lee-leung}, to put it in tune with \ref{p:gath-interp},
and more generally with the results of Section~\ref{s:YZ-gen}
below.

Given a smooth elliptic curve $E$, there are $\sigma_1 (2) = 1+2
=3$ morphisms of elliptic curves $E' \to E$ of degree $2$ (note that we
require that the origin is respected), as we have already
seen in \ref{p:ell-covers-enum}.
This implies that each of the $N^p _{1,1}$ elliptic curves $C$ in the
primitive linear system $|L|$ passing through a general point $x_1 \in
S$ gives via double covers of its normalization three genus $1$ stable
maps realizing the homology class $2[C]$, each contributing by $1$ to
the number $N^p_{1,2}$.

Lee and Leung deduce from this that $N_1^{4p-3}$ is the actual
number of physical elliptic curves in $|2L|$, meaning that it counts
each integral elliptic curve $C \in |2L|$ for $1$ and each $2C$ where
$C \in |L|$ is an integral elliptic curve for $1$ as well.
This is indeed a striking interpretation, although arguably
debatable. 

There is at any rate a phenomenon that prevents this interpretation to
be anything more than philosophical, namely that reducible curves
$C_0+C_1$, where $C_0$ (resp. $C_1$) is a rational (resp. elliptic)
integral curve in $|L|$, also contribute to the invariant
$N^p_{1,2}$. The two curves $C_0$ and $C_1$ intersect (transversely,
say) at $2p-2$ points $y_1,\ldots,y_{2p-2}$, and this gives $2p-2$
genus $1$ stable maps
\[
\P^1 \cup_{y_i} \bar C_1 \to S
\]
realizing the class $2L$ and passing through the appropriate fixed
point whenever $C_1$ does (the source is the transverse union of
the normalization $\P^1$ and $\bar C_1$ of $C_0$ and $C_1$,
attached at one
point lying in the preimages of one of the points $y_i$).


\subsection{The Yau--Zaslow formula for non-primitive classes}
\label{s:YZ-gen}

We now come to the general statement confirming \ref{p:gath-interp}
and recently proved by Klemm, Maulik, Pandharipande, and Scheidegger.

\paragraph{}
\label{p:GW0-K3}
Let $S$ be a $K3$ surface, and $L \in \Pic (S)$.
It follows from deformation invariance of reduced Gromov--Witten
integrals and the global Torelli theorem for $K3$ surfaces that the
integral 
$
\int _{[ \overline{M}_{0}(S,L)]^{\rm red}} 1
$
only depends on the self-intersection $L^2$ and the divisibility index
of $L$ in $\Pic (S)$
(the latter is
the largest integer
$m$ for which there exists $L' \in \Pic (S)$ such that
$L = m L'$).
We may thus make the following definition.

For all integers $p >0$ and $m \geq 1$, we let
\begin{equation*}
N^p _{0,m} :=
\int _{[ \overline{M}_{0}(S,mL)]^{\rm red}} 1
\end{equation*}
where $(S,L)$ is any primitively polarized $K3$ surface of genus $p$.

\paragraph{BPS states}
\label{p:bps}
Similar to what has been done in \ref{p:instanton}, and following the
insight of \ref{p:gath-interp}, we now define new invariants from the
$N^p_{0,m}$ of \ref{p:GW0-K3} above by applying the corrections
indicated by the Aspinwall--Morrison formula.
Let us formulate this in
terms of generating series as follows.
Given a positive integer $p$, set
\begin{equation}
\label{eq:gen-GW0}
F^p(v) := \sum _{m \geq 1} N^p_{0,m} \,v^m
\end{equation}
as a formal power series in the variable $v$.
Then the new set of invariants $n^p_{0,m}$ is uniquely determined by
the rewriting of the generating series as
\begin{equation}
\label{eq:gen-BPS0}
F^p(v) := \sum _{m \geq 1} n^p_{0,m} 
\biggl(\, \sum_{d>0} \frac 1 {d^3} \,v^{dm}
\biggr)
\end{equation}
(this is exactly the same modification as that of
\eqref{eq:instantons}).

Note that this is not mere makeshift reformulation. The
invariants $n^p_{0,m}$ are believed to count objects named BPS states
by the physicists, after Bogomol'nyi, Prasad, and Sommerfield,
and have been introduced by Gopakumar and Vafa. The
mathematical nature of these BPS states is however not clear yet.
In particular, it
should be possible to define the $n^p_{0,m}$ intrinsically, without
relying on the $N^p_{0,m}$; the relation \eqref{eq:gen-BPS0} would
then tie together these two sets of independently defined invariants.
See the enlightening survey \cite[\S~2$\frac 12$]{pt-13/2} for more
about this. 
There is moreover a physical meaning to the introduction of generating
series, but I will not discuss it.

\begin{theorem}[\cite{KMPS}]
\label{T:KMPS}
The genus $0$ invariants $n^p_{0,m} $ do not depend upon the divisibility
index, \ie  for all integers $m,p \geq 1$, one has
\begin{equation}\label{kmps}
n^p_{0,m} = n^{m^2p-m^2+1}_{0,1} = N^{m^2p-m^2+1}_0
\end{equation}
(the integer $p'={m^2p-m^2+1}$ is designed such that $(mL)^2=2p'-2$ if
$L^2=2p-2$).
\end{theorem}

Recall that $N^p_0$ was defined in section~\ref{S:YZ}; the second
equality in \eqref{kmps} is by definition of $n^p_{0,1}$ and $N^p_0$.
This statement was part of the Yau--Zaslow conjecture
\cite{YZ}. Together with Theorem~\ref{T:YZ}, which was also part of
the Yau--Zaslow conjecture, it implies that all the $n^p_{0,m}$'s may
be computed by means of formula~\eqref{eq:YZ}.
The set of relations \eqref{eq:gen-GW0} being triangular invertible,
this also gives all genus $0$ reduced Gromov--Witten invariants of
$K3$ surfaces.
Section~\ref{S:KMPS} below contains an overview of the proof given by
Klemm, Maulik, Pandharipande, and Scheidegger \cite{KMPS} of
Theorem~\ref{T:KMPS}.

%As we already noted in \ref{p:gath-interp},
The truly remarkable
feature of the invariants $n^p_{0,m}$ displayed by this statement is
that the number of rational curves of prescribed degree in an
algebraic $K3$ surface does not depend on the algebraic geometry of
the surface.

\paragraph{}
\label{p:still-not-enum}
In spite of formula~\eqref{eq:gen-BPS0} taking into account the
Aspinwall-Morrison multiple cover correction, the invariants
$n^p_{0,m}$ do not in general count the actual number of rational
curves in $|mL|$.

One reason for this is the existence of more non-reduced curves
with rational support than those taken in consideration in the
correction \eqref{eq:gen-BPS0}, namely curves with reducible support.
For instance let $m=3$ and consider two integral rational curves
$C_1,C_2$. Then $2C_1+C_2 \in |3L|$, and there are correspondingly
finitely many
% two for each of the $2p-2$ intersection points of $C_1$
% and $C_2$
positive-dimensional components of $\overline{M}_0(S,3L)$, the general
points of which correspond to stable maps
\[
\P^1 \cup_x \P^1 \to S
\]
with source a transverse union of two $\P^1$'s, consisting of a double
cover of $C_1$ on the first component and the normalization of $C_2$
on the other.
These certainly give an excess contribution to the invariant
$N^p_{0,3}$, which is not taken into account in the definition of
$n^p_{0,3}$.

Such problematic phenomena do not occur for $m \leq 2$, so that
$n^p_{0,1}$ is directly enumerative as was already noted in
Section~\ref{S:YZ}, and $n^p_{0,2}$ counts reduced rational curves in
the way described in Section~\ref{s:gathmann}.
It would be very interesting to relate $n^p_{0,m}$ to the number of
integral rational curves in $|mL|$ for $m \geq 3$.

% But one may certainly also consider rational curves in
% 3b of the type 2C_1+C_2 with C_1 and C_2 (integral) rational curves in
% the class b (by this I mean stable maps from a transverse union of two
% P^1's meeting at exactly one point, which map the first P^1 doubly to
% C_1, the second simply to C_2, and their unique intersection point to
% one of the points in C_1 \cap C_2), which I believe also give an
% excess contribution to the GW invariant of rational curves in 3b. 

There were, at least conjecturally, no such phenomena at work in the
case of the quintic threefold discussed in subsection~\ref{s:quintic},
as part~(iii) of the Clemens conjecture~\ref{c:clemens} asserts that
two integral rational curves in a general quintic threefold never
intersect.
In a surface, there is of course not enough space for two
curves to avoid each other, so we inevitably have to deal with the
aforementoined degenerate contributions.
% An important difference with the case of the quintic threefold
% discussed in subsection \ref{s:quintic} above is that for $K3$
% surfaces part~(iii) of the Clemens conjecture~\ref{c:clemens} does not
% hold, as there is of course not enough space in a surface for two
% curves to avoid each other.

The philosophy, as R.~Pandharipande communicated to me, is that
what the BPS numbers for $K3$ surfaces are virtually counting, are
rational curves in some perturbation of the twistor family of the $K3$
surface (a threefold, \cf\ref{p:sympl}). We shall consider in more
detail the close interplay between counting invariants for $K3$
surfaces and Calabi--Yau threefolds in the next Section~\ref{S:3fold}.



\section{Relations with threefold invariants}
\label{S:3fold}

It is already visible in the very foundation of the theory of
Gromov--Witten invariants for algebraic $K3$ surfaces developed by
Bryan--Leung \cite{BL}, see \ref{p:sympl}, that these invariants are
fundamentally attached to a threefold (even though the approach by
Maulik--Pandharipande \cite{MP}, see \ref{p:redGW}, 
bypasses this).
Another revealing evidence of the $3$-dimensional nature of these
invariants is the meaningful role played by the Aspinwall--Morrison in
the Yau--Zaslow statement discussed in subsection~\ref{s:YZ-gen}
above, a tool specifically designed for Calabi--Yau threefolds.
In this section we will try to describe this relation in a more
conceptual way.
It it wise to keep in mind the symplectic nature of Gromov--Witten
invariants throughout.


\subsection{Two obstruction theories}
\label{s:2obstr}

\paragraph{A threefold degenerate contribution}
\label{p:3fold-deg-contrib}
Let $V$ be a Calabi--Yau threefold. It follows from formula
\eqref{eq:vdim} that the virtual dimension of all spaces of stable maps 
is $0$ regardless of the genus.
This makes the following phenomenon happen.

Let $C_0 \subset V$ be a rational curve (smooth and
infinitesimally rigid, say). Its normalization $f: \P^1 \to V$
contributes regularly by $1$ to the integral
$\int _{[\overline{M}_0(V,[C_0])]^{\rm vir}} 1$.
But for any stable curve $C'$ of genus $g \geq 1$ we may obtain a
genus $g$ stable map realizing the class $[C_0]$ by attaching $C'$ to the
normalization of $C_0$ over a smooth point $x$, and letting
\[
f_{C',x}: \P^1 \cup_x C_0 \to V
\]
equal to $f$ along $\P^1$ and collapsing $C'$ to $x$.
This produces a positive dimensional moduli space of genus $g$ stable
maps which all have the same image $C_0 \subset V$; its contribution to
the Gromov--Witten invariant
$\int _{[\overline{M}_g(V,[C_0])]^{\rm vir}} 1$
must be computed via Hodge integrals over the moduli space of stable
curves of genus $g$, see below.
This has been studied by Faber and Pandharipande, see
\cite[\S~$1\frac 12$]{pt-13/2} and the references therein.

\paragraph{Curves in the twistor space of a $K3$}
\label{p:2obstr}
Let $S$ be a $K3$ surface, together with an algebraic class $\beta \in
H_2(S,\Z)$. We consider its twistor space $T \to {\bf S}^2$
described in \ref{p:sympl} above (we emphasize that this is a real
$6$-dimensional variety), and
denote by $\iota: S \hookrightarrow T$
the canonical inclusion of $S$. Since curves in $T$ can only appear
in the fibre $S$, we have the equality of moduli spaces of stable maps
\begin{equation*}
\overline{M}_g (T,\iota_* \beta)
= \overline{M}_g (S,\beta),
\end{equation*}
a priori only as sets but in fact as Deligne--Mumford stacks.
They come however with two different obstructions theories, hence also
with two different virtual classes. Gromov--Witten invariants on $T$
are related to those on $S$ 
(within the reduced theory for $K3$ surfaces, \cf \ref{p:redGW})
by the formula
\begin{equation}
\label{eq:hdg-int}
\int _{[\overline{M}_g (T,\iota_* \beta)] ^{\rm vir}} 1
\ =\ \int _{[\overline{M}_g (S,\beta)] ^{\rm red}} (-1)^g \lambda_g,
\end{equation}
where $\lambda_g$ stands for the top Chern class $c_g(\mathbf{E}_g)$
of the Hodge bundle $\mathbf{E}_g \to \overline{M}_g (S,\beta)$, whose
fibre over the stable map $f: C \to S$ is $H^0(C,\omega _C)$.

\paragraph{Hodge integrals}
It follows from the invariance of reduced Gromov--Witten invariants
under algebraic deformation and the global Torelli theorem for $K3$
surfaces that the right-hand side of \eqref{eq:hdg-int} depends only
on the self-intersection $\beta^2$ and the divisibility index of
$\beta$ as an algebraic class. We may thus formulate the following
definition.

For integers $g \geq 0$ and $p,m \geq 1$, let
\begin{equation}
\label{eq:bps0}
R^p _{g,m} :=
\int _{[ \overline{M}_{g}(S,mL)]^{\rm red}} (-1)^g \lambda_g
\end{equation}
where $(S,L)$ is any primitively polarized $K3$ surface of genus $p$,
and $\lambda_g$ is the top Chern class of the Hodge bundle as in 
\ref{p:2obstr} above.

This extends the definition of the invariants $N^p_{0,m}$ in
\ref{p:GW0-K3} above, in the sense that $N^p_{0,m} = R^p_{0,m}$
(note however that the invariants $N^p_{1,2}$ used in
subsection~\ref{s:lee-leung} do not coincide with the $R^p_{1,2}$).
For $g>0$, these invariants are certainly not counting curves on $S$;
rather, formula~\eqref{eq:hdg-int} tells us that they virtually give the
excess contribution of $S$ to the vertical Gromov--Witten theory of any
$K3$-fibred threefold in which it appears as a fibre. This philosophy
is put into concrete form by Theorem~\ref{T:MP} below.


\subsection{The Katz--Klemm--Vafa formula}

This is an extension of the Yau--Zaslow conjecture discussed in
Section~\ref{s:YZ-gen} above to the invariants $R^p_{g,m}$. It has
been proved by Pandharipande and Thomas \cite{PT-KKV}, 
see also \cite{PT-surveyKKV}.

\paragraph{BPS invariants}
\label{p:BPS}
It is admittedly better to organize the invariants $R^p_{g,m}$ in BPS form
as in \ref{p:bps}. We have now a clear justification for this, as we
have seen in Section~\ref{s:2obstr} above that these invariants
really count objects on threefolds.

We first let
\begin{equation*}
F^p(u,v) := \sum _{g \geq 0} \sum _{m>0}
R^p_{g,m} \, u^{2g-2} v^m
\end{equation*}
as formal power series in the two variables $u,v$
for all positive integers $p$.
One then defines new invariants $r^p_{g,m}$ for all integers $p,m>0$,
$g \geq 0$, by setting
\begin{align*}
F^p(u,v) &=  \sum _{m>0} \sum _{g \geq 0}
\, r^p _{g,m} u^{2g-2} 
\left( \, \sum _{d>0} \frac 1 d \left(
\frac {\sin d \frac u 2} {\frac u 2}
\right) ^{2g-2} v^{dm} 
\right) \\
&=
\begin{aligned}[t]
\sum _{m>0}
&\left( r^p_{0,m} u^{-2} 
\sum _{d>0} \Bigl(
\frac 1 {d^3} + \frac 1 {12d} u^2 + \frac d {240} u^4
+ \frac {d^3} {6048} u^6 + \frac {d^5} {172800} u^8 + \cdots
\Bigr) v ^{dm}
\right. \\
&+ r^p_{1,m} \sum _{d>0} \frac 1 d\, v^{dm} \\
&+ r^p_{2,m} u^2 \sum _{d>0} \Bigl(
d - \frac {d^3} {12} u^2 + \frac {d^5}{360} u^4
- \frac {d^7}{20160} u^6 + \frac {d^9}{1814400} u^8 + \cdots
\Bigr) v ^{dm} \\
&+ r^p_{3,m} u^4 \sum _{d>0} \Bigl(
d^3 - \frac {d^5}{6} u^2 + \frac {d^7}{80} u^4
- \frac {17d^9}{30240} u^6
+ \frac {31 d^{11}}{1814400} u^8
 + \cdots
\Bigr) v ^{dm} \\
& \left. \vphantom{\sum_m}
+ \cdots \right).
\end{aligned}
\end{align*}
The modifications for genus $g>0$ objects did not appear earlier in
this text.
Note that every object counted by $r^p_{g,m}$ contributes to the
invariants $R^p_{g',m}$ for all $g' \geq g$ (except when $g=1$), with
alternated sign if $g \geq 2$.
This is in accord with what the phenomenon described in 
\ref{p:3fold-deg-contrib}
suggests.


\begin{theorem}[Katz--Klemm--Vafa formula, \cite{PT-KKV}]
\label{T:KKV}
The invariants $r^p_{g,m}$ do not depend on the divisibility index,
meaning that one has
\begin{equation*}
r^p_{g,m} = r^{m^2p-m^2+1} _{g,1} = R^{m^2p-m^2+1} _g
\end{equation*}
for all integers $p,m >0$ and $g \geq 0$.

They are all determined by the formula
\begin{equation}\label{eq:KKV}
\sum_{p\geq 0} \sum_{g\geq 0} (-1)^g \, r^p_{g}
\,\bigl( y^{\frac{1}{2}} - y^{-\frac{1}{2}} \bigr)^{2g}
\, q^p =
\prod_{n\geq 1}\, \frac{1}{(1-q^n)^{20} (1-yq^n)^2 (1-y^{-1}q^n)^2},
\end{equation}
where we set $r^p_g:=r^p_{g,1}$
(and for convenience, $r^0_0=1$, and $r^0_g =0$ for all $g>0$).
\end{theorem}

Setting $y=1$ in the formula restricts to the invariants $r^p_0$, and
recovers the Yau--Zaslow formula of Theorem~\ref{T:YZ}.
As a first corollary, one gets that $r^p_g=0$ if $g>p$, and $r^p_p =
(-1)^p (p+1)$. The first values of $r^p_g$ are tabulated below.
\begin{center}
\begin{tabular}{|c|ccccc|}
\hline
\diagbox {$g$} {$p$} & 0 & 1  & 2 & 3 & 4 \\
\hline% \hline
$0$ & $1$ & $24$ & $324$ & 
$3200$ &$25650$  \\
1      &  & $-2$ & 
$-54$ & $-800$  & $-8550$      \\
2      & & & $3$ & 
$88$ & $1401$       \\
3      & &  & 
 & $-4$  & $-126$       \\
4      &  &  & 
 &   & 5       \\
       \hline
\end{tabular}
\captionof{table}{First values of $r^p_g$}
\end{center}



\subsection{Further Gromov--Witten integrals}
\label{s:furtherGW}

We close this section with a short discussion of further results about
Gromov--Witten integrals on $K3$ surfaces. They all come from
\cite{MPT}.

\paragraph{Hodge integrals with point insertions}
As a direct generalization of the invariants
$R^p _{g,m}$ from \eqref{eq:bps0}, one may
consider the integrals
\begin{equation*}
R^p _{g,k,m} :=
\int _{[ \overline{M}_{g,k}(S,mL)]^{\rm red}} (-1)^{g-k} \lambda_{g-k} \cup
\ev_1^* (\pt) \cup \cdots \cup \ev_k^* (\pt),
\end{equation*}
where $(S,L)$ is a primitive $K3$ surface of genus $p$,
$\Mbar_{g,k}(S,mL)$ is the moduli space of genus $g$
stable maps with $k$ marked points, and
$\lambda_i$ is the $i$-th Chern class of the Hodge bundle 
$\mathbf{E}_{g,k} \to \overline{M}_{g,k} (S,mL)$ as in \ref{p:2obstr}.

For \emph{primitive} classes on $K3$ surfaces, the following formula
was proved by Maulik, Pandharipande and Thomas \cite[Thm.~3]{MPT}:
\begin{multline}
\label{KKV-MPT}
% \sum_{g= 0}^{\infty} \sum_{h = 0}^{\infty}
% \Big\langle (-1)^{g-k} \lambda_{g-k} \tau_0(\mathsf{p})^{k}
% \Big\rangle^{S}_{g, h} u^{2g-2}
% q^{h-1}
% =\\ 
\quad
\sum_{g= 0}^{+\infty} \sum_{p = 0}^{+\infty}
R^p _{g,k,1} \, u^{2g-2} q^{p}
\ =
\\
q\,
\frac {(2\pi)^{12}} {u^{2} \Delta(q)} \cdot
\exp \left( \sum_{g=1}^{+\infty} u^{2g} \frac{B_{2g}}{g(2g)!} 
E_{g}(q) \right)
\cdot
\left( \sum_{m= 1}^{+\infty} q^{m} \sum_{d | m} \frac{m}{d} 
\big( \textstyle {2 \sin d \frac u 2 } \big)^{2}
\right)^{k}
\quad
\end{multline}
(notation is as in \ref{p:modular}).

Note that in the $k=0$ case, this contains nothing new with
respect to the formula given in Theorem~\ref{T:KKV}, as the expression
\eqref{KKV-MPT} may be deduced from \eqref{eq:KKV} using known
identities, see \cite[\S~5.4]{MPT}.


\paragraph{Descendent Gromov--Witten invariants}
So far, we have been essentially concerned with the reduced Gromov--Witten
invariants (see \ref{p:redGW})
\begin{equation*}
N_g (S,\beta) 
= \int _{[\Mbar_{g,g} (S,\beta)] ^{\rm red}} \ev_1^* (\pt) \cup \cdots
\cup \ev_g^* (\pt)
\end{equation*}
counting curves in the algebraic class $\beta \in H_2(S,\Z)$ on the $K3$
surface $S$ and passing through $g$ general fixed points.
It is of course possible to pull-back more general cohomology classes
$\gamma_i \in H^*(S,\Z)$ by the evaluation maps, thus encoding more
general incidence conditions than the passing through a given point
(although this is not really relevant for surfaces due to the
divisor axiom of Gromov--Witten theory).
Beware that when doing so one gets integrals that do depend on the
class $\beta$ itself, and not only on its self-intersection and
divisibility index, as classes in $H^2(S,\Z)$ are not monodromy
invariant.

A more sensible generalization is to integrate \emph{descendent
classes}. Let $\Mbar _{g,k} (S, \beta)$ be the moduli space of genus $g$
stable maps with $k$ marked points realizing the class $\beta$, and
$\ev_1,\ldots,\ev_k$ the corresponding evaluation maps
$\Mbar _{g,k} (S, \beta) \to S$.
For all $i=1,\ldots,k$, define the \emph{$i$-th cotangent line bundle}
$L_i$ to be the line bundle over 
$\Mbar_{g,k} (S, \beta)$ the fibre of which over the point $(f: C \to
S,p_1,\ldots,p_k)$ is the $\C$-line $\Omega_{C,p_i} ^1$.
The descendent classes on $\Mbar _{g,k} (S, \beta)$ are those gotten
from the Chern classes of these line bundles.

Let $\psi_i := c_1 (L_i) \in H^2\bigl( \Mbar _{g,k} (S, \beta), \Q
\bigr)$. For all cohomology classes $\gamma_1,\ldots,\gamma_k \in
H^*(S,\Z)$ and non-negative integers $n_1,\ldots,n_k$, we set
\begin{equation}
\label{eq:descGW}
\bigl\langle \tau_{n_1} (\gamma_1) \cdots \tau_{n_k} (\gamma_k)
\bigr\rangle ^{S,\beta} _g
:= \int _{[\Mbar _{g,k} (S, \beta)] ^{\rm red}} \psi_1^{k_1} \cup
\ev_1^* (\gamma_1) \cup \cdots \cup \psi_k^{k_k} \cup
\ev_k^* (\gamma_k)
\end{equation}
whenever the degree of the integrand equals the (real) dimension
$2g+2k$ of the reduced virtual class, and
$\bigl\langle \tau_{n_1} (\gamma_1) \cdots \tau_{n_k} (\gamma_k)
\bigr\rangle ^{S,\beta} _g :=0$ otherwise.
These integrals are called 
\emph{reduced descendent Gromov--Witten invariants}.

The geometric interpretation of the insertion of the classes $\psi_i$
is not straightforward; I refer to \cite{P-bourbaki} and
\cite{gathmann-habil} for some discussions about this. See however
\cite[Thm.~2.2.6]{gathmann-habil}, where descendent classes are used 
to define Gromov--Witten invariants of a projective manifold $X$
\emph{relative} to a smooth very ample hypersurface $Y$, \ie
invariants virtually counting curves in $X$ with prescribed tangency
conditions along $Y$.


\paragraph{Quasi-modularity}
The integrals \eqref{eq:descGW} for fixed integrand and fixed $g$ and
divisibility index of $\beta$ are expected to fit together as the
Fourier coefficients of a quasi-modular form, as in
Theorem~\ref{T:BL}.
Due to their dependency on the class $\beta$ and not only on its
numerical characters, this is formulated as follows.

Let $S$ be an arbitrarily fixed $K3$ surface possessing an elliptic
fibration $\pi:S \to \P^1$ and a section $E$ of $\pi$.
Call $\ste, \stf \in H_2(S,\Z)$ the classes of $E$ and the
fibres of $\pi$ respectively.
It follows from deformation invariance and the same 
standard degeneration argument as in the proof of Theorem~\ref{T:BL}
that any integral of the form \eqref{eq:descGW} on an algebraic $K3$
surface equals an integral of the same kind on $S$ with $\beta=a\ste +
b\stf$ for some non-negative integers $a,b$.
For all integers $g\geq 0$ and $m>0$, we set
\begin{equation*}
F_{g,m} ^S \bigl( \tau_{n_1} (\gamma_1) \cdots \tau_{n_k} (\gamma_k)
\bigr)
:= \sum_{n \geq 0} \bigl\langle \tau_{n_1} (\gamma_1) \cdots
\tau_{n_k} (\gamma_k) \bigr\rangle ^{S,m\ste+n\stf} _g
q^{m(n-m)}
\end{equation*}
as a formal power series in the variable $q$.


\begin{conjecture}
[Maulik and Pandharipande,
{\cite[Conj.~3]{P-survey}} and
{\cite[\S~7.5]{MPT}}]
The power series
$F_{g,m} ^S \bigl( \tau_{n_1} (\gamma_1) \cdots \tau_{n_k} (\gamma_k)
\bigr)$
is the Fourier expansion in $q$ of a quasi-modular form of level $m^2$
with pole at $q=0$ of order at most $m^2$.
\end{conjecture}

\noindent
(A quasi-modular form of level $N$ with possible pole at $q=0$ is by
definition an element of the $\C$-algebra generated by the Eisenstein
series $G_1$ (see \ref{p:modular}) and modular forms of level $N$;
recall in addition that a modular form of level $N$ is a form
satisfying the modular equation for transformations in the congruence
subgroup $\Gamma_0(N)$ consisting of elements of $\mathrm{PSL}_2 (\Z)$
congruent to the identity matrix modulo $N$).

\smallskip
For $m=1$, \ie for primitive classes, this was proved by Maulik,
Pandharipande and Thomas \cite[Thm.~4]{MPT}.
Note however that, even in the primitive case, there is no general
explicit formula for the modular form in question,
as far as I know.
Theorem~\ref{T:BL} provides particular instances of such a
formula.
At any rate, modularity strongly constrains the invariants and in
favorable cases enables one to compute them all (see \ref{p:B-KM} for
an example in a different context).


\medskip
We will only say the following
about the proofs of the results presented
in this section. A fundamental
ingredient for them is the use of other counting invariants than those
coming from Gromov--Witten theory, together with correspondence
theorems between the two. 
They are more algebraic in nature than Gromov--Witten invariants, and
more agile to study the problems we have been discussing.
These invariants virtually count \emph{stable pairs}; they were defined by
Pandharipande and Thomas, specifically for threefolds up to now. 
See \cite{pt-13/2} for a presentation.


\section{Noether--Lefschetz theory and applications}
\label{S:KMPS}

\subsection{Lattice polarized $K3$ surfaces and
Noether--Lefschetz theory}

In this subsection we define Noether--Lefschetz divisors in the moduli
spaces of lattice polarized $K3$ surfaces. While the version we will
use is the refined one of \ref{p:NLdivs-ref}, the elementary version
of \ref{p:NLdivs-elem} is needed to give a proper definition.

%\smallskip
Let $\bLK := U^{\oplus 3} \oplus E_8(-1)^{\oplus 2}$ be the $K3$
lattice (see, \eg \cite{bpv}). Throughout this subsection, we consider
a fixed lattice $\Lambda$ of rank $r$ and signature $(1,r-1)$, together
with a primitive embedding $\iota: \Lambda \hookrightarrow \bLK$ (the
embedding is \emph{primitive} if the corresponding quotient 
$\bLK/ i(\Lambda)$
is torsion-free).

\begin{definition}
Let $S$ be a $K3$ surface. A $\Lambda$-polarization on $S$ is a
primitive embedding
$j: \Lambda \hookrightarrow \Pic (S)$ such that
\begin{mycpctenum}[(i)]
\item there is a nef and big class in $j(\Lambda) \subset \Pic (S)$;
\item there exists an isometry $\phi: H^2(S,\Z) \to \bLK$ such that
$\phi \circ j = \iota$.
\end{mycpctenum}

A $\Lambda$-polarized $K3$ surface is a pair $(S,j)$ where $S$ is
a $K3$ surface and $j$ is a $\Lambda$-polarization on $S$.
\end{definition}

There exists a moduli space $\cK_\Lambda$ of $\Lambda$-polarized $K3$
surfaces, which may be constructed relying on the global Torelli
theorem  by adapting the method of \cite[Exp.~XIII, \S3]{palaiseau}.

\paragraph{} \label{p:latt-ext}
Define the discriminant of a rank $s$ lattice $L$ to be the signed
determinant
\[
\Disc (L):=
(-1)^{s-1} \det \bigl( 
\langle v_i,v_j \rangle \bigr)_{1 \leq i,j\leq s}
\]
where $(v_1,\ldots,v_s)$ is an integral basis of $L$
(the sign has been added to the usual definition so that
$\Disc (\Lambda) >0$); this does not depend on the choice of the basis.

Let $\bL$ be a rank $r+1$ lattice with an even symmetric
bilinear form, together with a primitive embedding 
$i: \Lambda \hookrightarrow \bL$. There is an invariant of the pair
$(\bL,i)$
called the {coset}, which is defined as follows.
Consider any vector $v \in \bL$ such that
$\bL = i(\Lambda) \oplus v$; the pairing with $v$ determines an
element $\ell_v \in \Lambda ^\vee$ in the lattice dual to $\Lambda$.
On the other hand, let $G_\Lambda:= \Lambda ^\vee / \Lambda$ be the
quotient of the injection $\Lambda \hookrightarrow \Lambda^\vee$
defined by the pairing on $\Lambda$;
it is an abelian group of order $\Disc (\Lambda)$. 
The \emph{coset}
$\delta$ of $(\bL,i)$ is the class of $\ell_v$ in $G_\Lambda/\pm$; it
does not 
depend on the choice of $v$.

Two pairs $(\bL,i)$ and $(\bL',i')$ as above are isomorphic 
(\ie there exists an isometry $\phi: \bL \to \bL'$ such that 
$\phi \circ i = i'$) if and only if the following two conditions
hold: (i) $\Disc (\bL) = \Disc(\bL')$, and (ii) $\delta(\bL,i) =
\delta (\bL',i')$.

\paragraph{Elementary Noether--Lefschetz divisors}
\label{p:NLdivs-elem}
The \emph{Noether--Lefschetz divisor}
$P_{\Delta,\delta}^\Lambda \subset \cK_\Lambda$
is the closure of the locus of $\Lambda$-polarized $K3$
surfaces $(S,j)$ such that $\Pic (S)$ has rank $r+1$ and discriminant
$\Delta$, and the coset $\delta(\Pic (S),j)$ equals $\delta$.

It follows from the Hodge index theorem that the divisor
$P_{\Delta,\delta}^\Lambda$ is empty when $\Delta \leq 0$.


\paragraph{Refined Noether--Lefschetz divisors}
\label{p:NLdivs-ref}
Let us now fix an integral basis $\bv _\Lambda =(v_1,\ldots,v_r)$ for
$\Lambda$,
and let $m \in \Z_{>0}$,
and $(p,\bd)= (p,d_1,\ldots,d_r) \in \Z^{r+1}$.
We want to define a Noether--Lefschetz divisor $D_{m,p,\bd} ^{\bv_\Lambda}
\subset \cK_\Lambda$ corresponding to $\Lambda$-polarized $K3$
surfaces $(S,j)$ with an extra class $\beta \in \Pic (S)$ of
divisibility index $m$ such that
$\langle \beta,\beta \rangle = 2p-2$, and
$\langle \beta,v_i \rangle = d_i$ for all $i=1,\ldots,r$.
The definition depends on the following cases: let
\begin{equation*}
\Delta^{\bv_\Lambda} _{p,\bd} :=
(-1)^{r} \begin{vmatrix}
\langle v_1,v_1 \rangle & \cdots 
& \langle v_1,v_r \rangle & d_1 \\
\vdots & \ddots & \vdots & \vdots \\
\langle v_r,v_1 \rangle & \cdots
& \langle v_r,v_r \rangle & d_r \\
d_1 & \cdots & d_r & 2p-2
\end{vmatrix};
\end{equation*}
{\setlength{\parindent}{0mm}
\begin{asparaitem}[---]
\item if $\Delta^{\bv_\Lambda} _{p,\bd} >0$, set 
\begin{equation*}
D_{m,p,\bd} ^{\bv_\Lambda} := 
\sum _{\Delta,\delta} \mu_{m,p,\bd} ^{\bv_\Lambda} (\Delta,\delta)
\cdot P^\Lambda _{\Delta,\delta}
\end{equation*}
where the sum runs over all $\Delta$ and $\delta$ such that there exists a
pair $(\bL,i)$ as in \ref{p:latt-ext} with $\Disc (\bL) = \Delta$ and
$\delta (\bL,i) = \delta$ (the pair $(\bL,i)$ is then unique up to
isomorphism),
and $\mu_{m,p,\bd} ^{\bv_\Lambda} (\Delta,\delta)$ is the number of
elements $\beta \in \bL$ having divisibility index $m$ and satisfying
$\langle \beta,\beta \rangle = 2p-2$ and
$\langle \beta,v_i \rangle = d_i$ for all $i=1,\ldots,r$.
Note that $\mu_{m,p,\bd} ^{\bv_\Lambda} (\Delta,\delta)$ may be $0$;
its non-vanishing implies that $\Delta$ divides
$\Delta^{\bv_\Lambda} _{p,\bd}$, so the above sum has only finitely
many terms. The condition $\Delta^{\bv_\Lambda} _{p,\bd} >0$ implies
that any $\beta$ such that $\langle \beta,\beta \rangle = 2p-2$ and
$\langle \beta,v_i \rangle = d_i$ for all $i$ does not belong to
$i(\Lambda)$; 
\item if $\Delta^{\bv_\Lambda} _{p,\bd} <0$, set 
$D_{m,p,\bd} ^{\bv_\Lambda} :=0$;
\item if $\Delta^{\bv_\Lambda} _{p,\bd} =0$ and $m=
\gcd(d_1,\ldots,g_r)$, let $D_{m,p,\bd} ^{\bv_\Lambda}$ be the divisor
associated to the dual of the Hodge line bundle 
$\cE \to \cK_\Lambda$ (the fibre of $\cE$ over the point $(S,i)$ is
$H^{2,0}(S)$);
\item if $\Delta^{\bv_\Lambda} _{p,\bd} =0$ and $m \neq
\gcd(d_1,\ldots,g_r)$, set 
$D_{m,p,\bd} ^{\bv_\Lambda} :=0$.
\end{asparaitem}
}


\subsection{Invariants of families of lattice polarized $K3$
surfaces}

\paragraph{Families of lattice polarized $K3$ surfaces}
\label{def:pol-fam}
Let $\iota: \Lambda \hookrightarrow \bLK$ be a primitive embedding of
a lattice $\Lambda$ of rank $r$ and signature $(1,r-1)$.
A
\emph{1-parameter family of $\Lambda$-polarized $K3$ surfaces}
is a smooth
family $\pi: X \to C$ of $K3$ surfaces equipped with line bundles
$L_1,\ldots,L_r$ on $X$ such that:
\begin{mycpctenum}[(i)]
\item $X$ is a compact $3$-dimensional complex manifold (not
  necessarily algebraic), $C$ is a complete smooth complex curve, and
  $\pi$ is a holomorphic submersion;
\item for all $t\in C$, the fibre $X_t$ of $\pi$ over $t$ is a
(smooth) $K3$ surface; 
\item there exists a linear combination $L^\pi$ of the holomorphic
line bundles $L_i$ on $X$, the restriction of which to every fibre of
$\pi$ is nef and big;
\item \label{pol-fam-basis}
there exists an integral basis $(v_1,\ldots,v_r)$ of $\Lambda$
such that for all $t \in C$, the map $j_t: \Lambda \to \Pic X_t$
defined by 
$v_i \mapsto L_{i,t}$ (the restriction of $L_i$ to $X_t$) is a
$\Lambda$-polarization of $X_t$.
\end{mycpctenum}

\medskip
For the remainder of this subsection, we consider
a $1$-parameter family of $\Lambda$-polarized $K3$
surfaces
$(\pi: X \to C, L_1,\ldots,L_r)$
as in \ref{def:pol-fam} above.

\paragraph{Noether--Lefschetz numbers}
\label{p:NLnum}
Let $m \in \Z_{>0}$ and $(p,\bd)=(p,d_1,\ldots,d_r) \in
\Z^{r+1}$. 
The \emph{Noether--Lefschetz number}
$\NL^\pi _{m,p,\bd}$ is defined as
\begin{equation*}
\NL^\pi _{m,p,\bd} :=
\int _C f_\pi^* \bigl(D_{m,p,\bd} ^{\bv_\Lambda}\bigr),
\end{equation*}
where $f: C \to \cK_\Lambda$ is the morphism corresponding to
$(\pi: X \to C, L_1,\ldots,L_r)$
by the universal property of $\cK_\Lambda$, and $\bv_\Lambda$ is the
integral basis of $\Lambda$ defined by $(L_1,\ldots,L_r)$ via
point~\eqref{pol-fam-basis} of \ref{def:pol-fam}.

Note that this is a classical intersection product (\ie there is no
need to define a virtual class), although it may be given by an excess
formula in case the image $f_\pi(C)$ is fully contained in the divisor 
$D_{m,p,\bd} ^{\bv_\Lambda}$.

\paragraph{Gromov--Witten invariants for vertical curve classes}
Although it may not be a projective variety, the total space $X$
carries a $(1,1)$-form $\omega_\pi$ which is Kähler on the fibres of
$\pi$; this is sufficient to define a Gromov--Witten theory for
non-zero \emph{vertical} classes $\gamma \in H_2(X,\Z)^\pi$,
\ie classes $\gamma \in H_2(X,\Z)$ such that $\pi_*(\gamma)=0$
(see \cite[\S2.1]{MP} for details).

In this theory,
the moduli spaces of genus $g$ stable maps $\overline{M}_g(X,\gamma)$
all have virtual dimension $0$,
and we have a set of invariants
\begin{equation*}
N^X_{g,\gamma} := \int_{[\overline{M}_g(X,\gamma)]^{\rm vir}} 1
\end{equation*}
for non-zero {vertical} classes $\gamma$.
We consider the invariants $n^X_{g,\gamma}$ obtained
from the $N^X_{g,\gamma}$ by applying the BPS corrections packaged in the
formula of \ref{p:BPS}: we let
\begin{equation*}
F^X (u,v) := \sum _{g \geq 0} 
\ \sum _{0 \neq \gamma \in H_2(Z,\Z)^\pi}
N^X_{g,\gamma} \, u ^{2g-2} v^\gamma
\end{equation*}
as a formal power series in the variables $u,v$, where the powers of
$v$ are indexed by $H_2(Z,\Z)^\pi$, and set
\begin{equation*}
F^X (u,v) := \sum _{g \geq 0} 
\ \sum _{0 \neq \gamma \in H_2(Z,\Z)^\pi}
\, n^X_{g,\gamma} \, u^{2g-2} 
\left( \, \sum _{d>0} \frac 1 d \left(
\frac {\sin d \frac u 2} {\frac u 2}
\right) ^{2g-2} v^{d\gamma} 
\right).
\end{equation*}
Finally, for a non-zero multidegree $\bd =(d_1,\ldots,d_r) \in
\Z^r$, we let $n^X_{g,\bd}$ be the invariant counting genus $g$ stable
maps in vertical classes of degree $d_1,\ldots,d_r$ with respect to 
$L_1,\ldots,L_r$ respectively, \ie
\begin{equation}
\label{eq:vert-deg}
n^X_{g,\bd} := 
\sum _{\gamma \in H_2(X,\Z)^\pi:\ 
\int_\gamma L_i = d_i}
n^X_{g,\gamma}.
\end{equation}

\paragraph{Reduced Gromov--Witten invariants of $K3$ fibres}
We also consider the invariants $r^p_{g,m}$ for $K3$ surfaces which
have been defined in \ref{p:BPS}; 
recall that they are the reduced Hodge integrals \eqref{eq:bps0} put in
BPS form.
Note that
we need to maintain the dependency on the divisibility index $m$,
because Theorem~\ref{T:MP} below is needed for the proof of the
independence on $m$ conjectured by Yau--Zaslow.

%\bigskip
A multidegree $\bd =(d_1,\ldots,d_r) \in \Z^r$ is positive with
respect to $L^\pi$ if for any line bundle $M$ on some fibre $X_t$ of
$\pi$,  
$(M,L_{i,t})=d_i$ for all $i$ implies $(M,L^\pi)>0$;
since $L^\pi$ is a linear combination of the $L_i$, this is an
elementary linear algebraic condition. 

\begin{theorem}[\cite{MP}]
\label{T:MP}
Let $\bd =(d_1,\ldots,d_r) \in \Z^r$ be  a multidegree
which is positive with
respect to $L^\pi$.
Then
\begin{equation}
\label{eq:MP}
n^X_{g,\bd} =
\sum _{p=0}^{+\infty} \sum_{m=1}^{+\infty}
r^p _{g,m} \cdot 
\NL^\pi _{m,p,\bd}.
\end{equation}
\end{theorem}

\noindent
(This is stated in \cite{MP} in the $r=1$ case
($\ie \bd \in \Z$), but as
noted in \cite{KMPS} the same proof goes through in general).

\medskip
The philosophy behind this relation is rather natural, and ought to be
compared to the discussion of Section~\ref{s:2obstr} above.
Consider the
genus $g=0$ case for simplicity; then the invariant $n^X_{0,\bd}$
counts vertical rational curves in $X$ of prescribed degrees with
respect to $L_1,\ldots,L_r$, and these are virtually in finite number.
There are on the other hand finitely many members of the family $\pi$
with algebraic divisor classes of the prescribed degrees with respect
to $L_1,\ldots,L_r$, each of which provides a finite number of
rational curves. The theorem morally says that the number of rational
curves in $X$ is the sum of these isolated contributions from the
fibres.

Of course the actual story is more complicated than this, if only
because of the existence of $1$-dimensional families of rational
curves on $X$, coming from finitely many rational curves in \emph{all}
$K3$ members of the family (which all have algebraic divisor classes,
as they are $\Lambda$-polarized), in spite of the virtual dimension
being $0$.
In other words, a Calabi-Yau threefold $X$ as in Theorem~\ref{T:MP}
above is far from satisfying the same properties than the
perturbations of the twistor families of algebraic $K3$ surfaces
on which BPS numbers are supposed to count curves.




\subsection{Application to the Yau--Zaslow conjecture}
\label{s:KMPSpf}

In this subsection we give an outline of the proof by
Klemm, Maulik, Pandharipande, and Scheidegger of the Yau--Zaslow
conjecture (Theorem~\ref{T:KMPS} above).
Recall that the invariants $r^p_{g,m}$ being invariant under algebraic
deformations of the $K3$ surface, it is enough to prove the result for
our favourite $K3$ surface. These invariants for certain elliptic $K3$
surfaces are expressed by means of the relation~\eqref{eq:MP}
for a particular family.

\paragraph{The $STU$ model}
\label{p:STU}
The central character of the proof is a smooth projective Calabi--Yau
$3$-fold $X$, known as the $STU$ model
and coming from physics (quoting \cite{KMPS}: the letter $S$ stands for
the dilaton and $T$ and $U$ label the torus moduli in the heterotic
string).
It is contructed as an anticanonical section of
a smooth projective toric $4$-fold $Y$ defined by an explicit fan in
$\Z^4$. 

The variety $X$ has the structure of a fibration $\pi: X \to \P^1$,
the general fibre of which is a smooth $K3$ surface, itself with an
elliptic fibration. It comes with two line bundles $L_1,L_2 \to X$,
defining a $\Lambda$-polarization on the family $\pi: X \to \P^1$
(leaving aside the fact that there are inevitably singular members),
where $\Lambda$ is the lattice with intersection form
\[
\begin{pmatrix}
0 & 1 \\
1 & 0 
\end{pmatrix}.
\]

The family $\pi$ has the shape of a Lefschetz pencil, in particular
each of its singular members has a unique ordinary double point as its
only singularity.
One may thus build an actual family $\tilde \pi: \tilde X \to C$ of
$\Lambda$-polarized $K3$ surfaces from $\pi$ as follows.
One first performs a base change by $t \mapsto t^2$ around each
singular member; to do so, one considers the $2:1$ covering $\epsilon: C
\to \P^1$ with branch divisor $\Disc (\pi)$, the set of points above
which $\pi$ fails to be smooth, and let $\pi^\flat: X^\flat \to C$ be
the family obtained from $\pi$ by applying the base change $\epsilon: C
\to \P^1$.
The new total space $X^\flat$ is singular, precisely it has an
ordinary $3$-fold double point at each singular point of a fibre
(analytically locally around such a point, $X$ is defined by the
equation $x^2+y^2+z^2=t$ in a $4$-dimensional complex ball, hence
$X^\flat$ is defined by $x^2+y^2+z^2=t^2$).
One then chooses for $\tilde X$ any small resolution of all these
singularities: this may be understood as first blowing-up once all
singular points, and then contracting one ruling of each exceptional
divisor (they are all smooth quadric surfaces). This has the effect
of replacing each fibre of $X^\flat$ by its minimal model.

One may determine the number of singular members of $\pi$ by the same
topological Euler characteristic computation as in
Section~\ref{s:pencil}. The Euler number $e(X)$ is found to be
$-480$ by toric intersection computations in the $4$-fold $Y$, hence
the number of singular fibres equals
\begin{equation*}
e(K3)\cdot e(\P^1) -e(X) = 528
\end{equation*}
($e(K3)$ denotes the common Euler number of all $K3$ surfaces, \ie $24$).


\paragraph{Modularity for Noether--Lefschetz numbers}
\label{p:B-KM}
It is a stunning application of a theory developed by Borcherds and
Kudla--Millson 
(see \cite{MP,KMPS} and the references therein) that the
Noether--Lefschetz numbers of a family of $\Lambda$-polarized $K3$
surfaces fit into a vector valued modular form.

In order to state this precisely,
let us return to the setup of \ref{p:NLnum} for a moment
(see \cite[\S~4]{MP} for a complete treatment).
One may define divisors $D_{p,\bd} ^{\bv_\Lambda}$ and 
numbers $\NL^\pi _{p,\bd}$ by dropping the requirement on the
divisibility index $m$ in \ref{p:NLdivs-ref}.
It is an elementary result \cite[Lemma~1]{KMPS} that the full set of
the numbers $\NL^\pi _{p,\bd}$ determine the refined
Noether--Lefschetz numbers $\NL^\pi _{m,p,\bd}$.
Let $\Mp_2(\Z)$ be the metaplectic double cover of $\SL_2(\Z)$. There
is a canonical representation 
\begin{equation*}
\rho_\Lambda ^*: \Mp_2(\Z) \to \End \bigl( \C[G_\Lambda] \bigr)
\end{equation*}
associated to $\Lambda$ (recall that $G_\Lambda = \Lambda^\vee /
\Lambda$). 

\begin{theorem}[Borcherds, Kudla--Millson, Maulik--Pandharipande]
\label{T:B-KM}
There exists a vector-valued modular form
\begin{equation*}
\Phi ^\pi (q) 
= \sum _{\gamma \in G_\Lambda} \Phi ^\pi_\gamma (q) \, u^\gamma
\in \C[[q ^{\frac 1 {2 \Disc \Lambda}} ]] \otimes \C[G_\Lambda]
\end{equation*}
of weight $\frac {22-r} 2$ and type $\rho_\Lambda ^*$,
such that the Noether--Lefschetz number $\NL^\pi _{p,\bd}$ is the
coefficient of $\Phi ^\pi _\gamma$ in
$q$ to the power
$\frac {\Delta ^{\bv_\Lambda} _{p,\bd}} {2 \Disc \Lambda}$,
% \[
% q ^{\frac {\Delta ^{\bv_\Lambda} _{p,\bd}} {2 \Disc \Lambda}},
% \]
where $\gamma \in G_\Lambda$ is any of the two liftings of the coset
$\delta ^{\bv_\Lambda} _{p,\bd} \in G_\Lambda/\pm$ represented by the linear
functional
$v_i \mapsto d_i$.
\end{theorem}

%\smallskip
Taking advantage of the strong structure results for modular forms,
Maulik and Pandharipande are able to use this theorem to derive
explicitly the Noether--Lefchetz numbers of classical families of $K3$
surfaces of genus $2 \leq p \leq 5$ (\ie double planes and complete
intersection $K3$'s).
A similar calculation is carried out in \cite{KMPS} for the $STU$
family, as one of the key steps in the proof of the Yau--Zaslow
conjecture.

\paragraph{}
Let us now return to the setup of \ref{p:STU}.
Theorem~\ref{T:B-KM} tells that the Noether--Lefschetz numbers of the
family $\tilde \pi: \tilde X \to C$ are the Fourier coefficients of a
scalar modular form of weight $10$. The vector space of such forms has
dimension $1$ and is generated by the Eisenstein series
\begin{equation*}
E_{5} (q) = E_2(q) E_3(q) = 
1 - 264 \sum _{n=1} ^{+\infty} \sigma_9(n) q^n
\end{equation*}
\cite[\S~VII.3.2]{serre-arithmetique} (notation as in
\ref{p:modular}).
It follows that it is enough to know one Noether--Lefschetz number to
determine the full modular form, and since we do know one of them,
namely the number $528$ of singular members of the $STU$ family, one
obtains that the number $\NL^{\tilde \pi} _{p,d_1,d_2}$ is the
coefficient in $q$ to the power
$\frac 1 2 \Delta (p,d_1,d_2)$
of the modular form $-4 E_2(q) E_3(q)$, where 
\begin{equation*}
\Delta (p,d_1,d_2) =
\begin{vmatrix}
0 & 1 & d_1 \\
1 & 0 & d_2 \\
d_1 & d_2 & 2p-2
\end{vmatrix}.
\end{equation*}


\paragraph{Mirror symmetry}
\label{p:mirror}
The $STU$ model $X$ being an anticanonical section of a smooth
semi-positive toric variety, its genus $0$ Gromov--Witten invariants
are known by mathematically proven mirror symmetry results.
This gives the corresponding invariants of $\tilde X$, the latter
being twice those of $X$ \cite[\S~5.2]{MP}.

Precisely, Givental has proven the relation of the genus $0$
Gromov--Witten invariants of $X$ by mirror transformation to
hypergeometric solutions of the Picard--Fuchs equations of the
Batyrev--Borisov mirror, see \cite{MP,KMPS} and the references
therein. This gives the following formula of Klemm--Mayr--Lerche
\cite[Prop.~5]{KMPS}
\begin{equation}
\label{eq:KML}
\sum _{(d_1,d_2) \in \mathcal P}
(d_2)^3 N_{0,(d_1,d_2)}^X\, q_1^{d_1} q_2 ^{d_2}
= -2
+2\, \frac {E_2(q_1) E_3(q_1)} { (2\pi) ^{-12} \Delta(q_1)}\,
\frac {E_2(q_2)} {j(q_1)-j(q_2)},
\end{equation}
where 
\begin{equation*}
j(q):= 1728\, \frac {\bigl(60G_2(q) \bigr)^3} {\Delta(q)}
= (2\pi)^{12} \frac {E_2(q)^3} {\Delta(q)} 
= \frac 1 q + 744 + 196884q + \cdots
\end{equation*}
(notation as in \ref{p:modular})
is the normalized $j$ function,
$\mathcal P = \bigl \{ (d_1,d_2) \neq (0,0):
d_1 \geq 0,
d_1 \geq -d_2
\bigr \}$,
and $N^X_{0,(d_1,d_2)}$ is defined by formula \eqref{eq:vert-deg}
from the various $N^X _{0,\gamma}$, $\gamma \in H_2(X,\Z)^\pi$.

\paragraph{Conclusion: the Harvey--Moore identity}
\label{p:harvey-moore}
Using the fact that the lattice $\Lambda$ has rank $2$,
Klemm--Maulik--Pandharipande--Scheidegger then show 
that the invariants $r^p_{0,m}$ are uniquely determined by the
relations \eqref{eq:MP} 
for the family $\tilde \pi: \tilde X \to C$,
and the numbers 
$n ^{\tilde X} _{0,(d_1,d_2)}$ and 
$\NL ^{\tilde \pi} _{m,p,(d_1,d_2)}$
\cite[Prop.~3]{KMPS}.
The two latter sets of numbers being known by the results of
\ref{p:B-KM} and \ref{p:mirror}, it is therefore enough,
in order to end the proof of Theorem~\ref{T:KMPS},
to show that the numbers $r^p_{0,m}$ predicted by the Yau--Zaslow
conjecture (\ie $r^p_{0,m} = r^{m^2p -m^2+1}_{0,1}$ together with the
formula of 
\ref{T:YZ} giving the $r^p_{0,1}$'s) indeed fit in the relations
\eqref{eq:MP}.
This takes the form of an identity between modular forms: 
let
\begin{equation*}
f(z) := 
\frac {E_2(z) E_3(z)} { (2\pi) ^{-12} \Delta(z)}
= \sum _{n=-1} ^{+\infty} c(n) q^n,
\quad q=e^{2\pi iz};
\end{equation*}
what has to be proven is
\begin{equation*}
\frac {f(z_1) E_2(z_2)} {j(z_1)-j(z_2)}
= \frac {q_1} {q_1-q_2} 
+ E_2(z_2)
-\sum_ {d,k,l >0} l^3 c(kl)\, q_1 ^{kd} q_2 ^{ld}.
\end{equation*}
This is the Harvey--Moore identity,
which has been proven by Zagier, see \cite[\S~4.2]{KMPS}.




\begin{references}

\begin{thebibliography}[Chapters in this Volume\footnote
  {see \url{https://www.math.univ-toulouse.fr/~tdedieu/\#enumTV}}]{II}

\bibitem[\tref{02.edoardo}]{02.edoardo}
Th.~Dedieu and E.~Sernesi, \emph{Deformations of curves on surfaces}.

% \bibitem{filippo-chap}
% F.~Viviani, \emph{Introduction to {G}romov--{W}itten invariants}, chapter in
%   the present volume.

\bibitem[\tref{13.th-classic}]{13.th-classic}
  Th.~Dedieu,
  \emph{Some classical formul{\ae} for curves and surfaces}.

\bibitem[\tref{14.th-vainsencher}]{14.th-vainsencher}
  Th.~Dedieu,
  \emph{Node polynomials for curves on surfaces}.

\bibitem[\tref{12.fra-goettsche}]{12.fra-goettsche}
  F.~Bastianelli and Th.~Dedieu,
  \emph{The G\"ottsche conjecture
  and the G\"ottsche--Yau--Zaslow formula}.

\end{thebibliography}

\begin{thebibliography}[External references]{10}

\bibitem{ballico-fontanari}
E.~Ballico {\normalfont \smfandname} C.~Fontanari,
\emph{Finiteness of rational curves of degree 12 on a general quintic
  threefold},
Pure Appl. Math. Q. {\bf 11} (2015), no.\ 4, 537--557.
%preprint  arXiv:1607.07994.

\bibitem{bpv}
W.~P. Barth, K.~Hulek, C.~A.~M. Peters {\normalfont \smfandname} A.~Van~de Ven,
  \emph{Compact complex surfaces}, second \smfedname, Ergebnisse der Mathematik
  und ihrer Grenzgebiete 3. Folge, vol.~4, Springer-Verlag, Berlin, 2004.

\bibitem{beauville-c1}
A.~Beauville,
\emph{Variétés k\"ahleriennes dont la première classe de Chern est
  nulle},
J. Differential Geom. {\bf 18} (1983), no.~4, 755--782.

\bibitem{beauville-counting}
\bysame , \emph{Counting rational curves on {$K3$} surfaces}, Duke Math. J.
  \textbf{97} (1999), no.~1, 99--108.

\bibitem{123}
J.~H. Bruinier, G.~van~der Geer, G.~Harder {\normalfont \smfandname} D.~Zagier,
  \emph{The 1-2-3 of modular forms}, Universitext, Springer-Verlag, Berlin,
  2008, Lectures from the Summer School on Modular Forms and their Applications
  held in Nordfjordeid, June 2004, Edited by Kristian Ranestad.

\bibitem{BL}
J.~Bryan {\normalfont \smfandname} N.~C. Leung, \emph{The enumerative geometry
  of {$K3$} surfaces and modular forms}, J. Amer. Math. Soc. \textbf{13}
  (2000), no.~2, 371--410 (electronic).

\bibitem{CdGP}
P.~Candelas, X.~C. de~la Ossa, P.~S. Green {\normalfont \smfandname} L.~Parkes,
  \emph{A pair of {C}alabi-{Y}au manifolds as an exactly soluble superconformal
  theory}, Nuclear Phys. B \textbf{359} (1991), no.~1, 21--74.

\bibitem{chen-10}
X.~Chen, \emph{A simple proof that rational curves on {$K3$} are nodal}, Math.
  Ann. \textbf{324} (2002), no.~1, 71--104.

\bibitem{ethan11}
E.~Cotterill, \emph{Rational curves of degree 11 on a general quintic 3-fold},
  Q. J. Math. \textbf{63} (2012), no.~3, 539--568.

\bibitem{cox-katz}
D.~A. {Cox} {\normalfont \smfandname} S.~{Katz}, \emph{{Mirror symmetry and
  algebraic geometry}}, Providence, RI: American Mathematical Society, 1999.

\bibitem{dalmeida}
J.~D'Almeida, \emph{Courbes rationnelles de degr\'e 11 sur une hypersurface
  quintique g\'en\'erale de {$\mathbf{P}^4$}}, Bull. Sci. Math. \textbf{136}
  (2012), no.~8, 899--903.

\bibitem{DS15-10}
\Th.~Dedieu {\normalfont \smfandname} E.~Sernesi, \emph{Equigeneric and
  equisingular families of curves on surfaces},
Publ. Mat. {\bf 61} (2017), no.\ 1, 175--212.

\bibitem{diaz-harris}
S.~Diaz {\normalfont \smfandname} J.~Harris, \emph{Ideals associated to
  deformations of singular plane curves}, Trans. Amer. Math. Soc. \textbf{309}
  (1988), no.~2, 433--468.

\bibitem{fgv}
B.~{Fantechi}, L.~{G\"ottsche} {\normalfont \smfandname} D.~{van Straten},
  \emph{{Euler number of the compactified Jacobian and multiplicity of rational
  curves}}, {J. Algebr. Geom.} \textbf{8} (1999), no.~1, 115--133.

\bibitem{fulton-harris}
W.~Fulton {\normalfont \smfandname} J.~Harris, \emph{Representation theory},
  Graduate Texts in Mathematics, vol.~129, Springer-Verlag, New York, 1991, A
  first course, Readings in Mathematics.

\bibitem{gathmann-habil}
A.~Gathmann, \emph{{Gromov-Witten invariants of hypersurfaces}}, Habilitation
  thesis, TU Kaiserslautern, 2003.

\bibitem{gathmann-conics}
\bysame , \emph{{The number of plane conics that are five-fold tangent to a
  given curve}}, {Compos. Math.} \textbf{141} (2005), no.~2, 487--501.

\bibitem{godement}
  R.~Godement,
  \emph{Topologie algébrique et théorie des faisceaux},
  Publ. Inst. Math. Univ. Strasbourg, No. 13,
  Hermann, Paris, 1958.

\bibitem{goettsche-pandharipande}
L.~G{\"o}ttsche {\normalfont \smfandname} R.~Pandharipande, \emph{The quantum
  cohomology of blow-ups of {${\bf P}^2$} and enumerative geometry}, J.
  Differential Geom. \textbf{48} (1998), no.~1, 61--90.

\bibitem{goettsche-betti-nbrs}
L.~G{\"o}ttsche, \emph{The {B}etti numbers of the {H}ilbert scheme of points on
  a smooth projective surface}, Math. Ann. \textbf{286} (1990), no.~1-3,
  193--207.

\bibitem{goettsche-conj}
\bysame , \emph{A conjectural generating function for numbers of curves on
  surfaces}, Comm. Math. Phys. \textbf{196} (1998), no.~3, 523--533.

\bibitem{huybrechts-diffeo}
D.~Huybrechts, \emph{Compact hyper-{K}\"ahler manifolds: basic results},
  Invent. Math. \textbf{135} (1999), no.~1, 63--113.

\bibitem{KMPS}
A.~{Klemm}, D.~{Maulik}, R.~{Pandharipande} {\normalfont \smfandname}
  E.~{Scheidegger}, \emph{{Noether-Lefschetz theory and the Yau-Zaslow
  conjecture}}, {J. Am. Math. Soc.} \textbf{23} (2010), no.~4, 1013--1040.

\bibitem{lee-leung-elliptic}
J.~Lee {\normalfont \smfandname} N.~C. Leung, \emph{Counting elliptic curves in
  {$K3$} surfaces}, J. Algebraic Geom. \textbf{15} (2006), no.~4, 591--601.

\bibitem{qing-liu}
Q.~{Liu}, \emph{{Algebraic geometry and arithmetic curves, transl. by R.
  Ern\'e}}, Oxford: Oxford University Press, 2006, paperback new edition.

\bibitem{MPT}
D.~{Maulik}, R.~{Pandharipande} {\normalfont \smfandname} R.~{Thomas},
  \emph{{Curves on $K3$ surfaces and modular forms}}, {J. Topol.} \textbf{3}
  (2010), no.~4, 937--996.

\bibitem{maulik-homfly}
D.~Maulik, \emph{Stable pairs and the {HOMFLY} polynomial}, Invent. Math.
  \textbf{204} (2016), no.~3, 787--831.

\bibitem{MP}
D.~{Maulik} {\normalfont \smfandname} R.~{Pandharipande}, \emph{{Gromov-Witten
  theory and Noether-Lefschetz theory}}, in \emph{{A celebration of algebraic
  geometry. A conference in honor of Joe Harris' 60th birthday, Harvard
  University, Cambridge, MA, USA, August 25--28, 2011}}, Providence, RI:
  American Mathematical Society (AMS); Cambridge, MA: Clay Mathematics
  Institute, 2013, 469--507.

\bibitem{morelli}
A.~Morelli, \emph{Un'osservazione sulle singolarit\`a delle trasformate
  birazionali di una curva algebrica}, Rend. Accad. Sci. Fis. Mat. Napoli (4)
  \textbf{29} (1962), 59--64.

\bibitem{mukai-symplectic}
S.~Mukai, \emph{Symplectic structure of the moduli space of sheaves on an
  abelian or {$K3$} surface}, Invent. Math. \textbf{77} (1984), no.~1,
  101--116.

\bibitem{oblomkov-yun}
A.~Oblomkov {\normalfont \smfandname} Z.~Yun, 
\emph{The cohomology ring of certain compactified Jacobians},
preprint arXiv:1710.05391.

\bibitem{pt-13/2}
R.~Pandharipande {\normalfont \smfandname} R.~P. Thomas, \emph{13/2 ways of
  counting curves}, in \emph{Moduli spaces}, London Math. Soc. Lecture Note
  Ser., vol.~411, Cambridge Univ. Press, Cambridge, 2014, 282--333.

\bibitem{P-survey}
R.~Pandharipande, \emph{Maps, sheaves, and {$K3$} surfaces},
Clay Lect. Notes,
Oxford University Press, Oxford, 2017, 159–185.
%prepublication arXiv0808.0253.

\bibitem{P-bourbaki}
\bysame , \emph{Rational curves on hypersurfaces (after {A}. {G}ivental)},
  Ast\'erisque (1998), no.~252, Exp.\ No.\ 848, 5, 307--340, S{\'e}minaire
  Bourbaki. Vol. 1997/98.

\bibitem{PT-surveyKKV}
R.~Pandharipande {\normalfont \smfandname} R.~P. Thomas,
\emph{{Notes on the proof of the KKV conjecture}},
Surv. Differ. Geom., {\bf 21}
International Press, Somerville, MA, 2016, 289--311.
% preprint arXiv:1411.0896.

\bibitem{PT-KKV}
\bysame ,
\emph{{The Katz-Klemm-Vafa conjecture for K3 surfaces}},
Forum Math. Pi {\bf 4} (2016), e4, 111 pp.
% preprint arXiv:1404.6698.

\bibitem{palaiseau}
{S\'eminaire Palaiseau Oct. 1981--Jan. 1982}, \emph{G\'eom\'etrie des surfaces
  {$K3$}: modules et p\'eriodes}, Ast{\'e}risque, vol.~126, Soci\'et\'e
  Math\'ematique de France, Paris, 1985.

\bibitem{edoardo}
\bysame , \emph{Deformations of algebraic schemes}, 
Grundlehren der Mathematischen Wissenschaften,
% [Fundamental Principles of Mathematical Sciences],
vol.~334, Springer-Verlag, Berlin, 2006.

\bibitem{serre-arithmetique}
J.-P. Serre, \emph{Cours d'arithm\'etique}, Collection SUP: ``Le
  Math\'ematicien'', vol.~2, Presses Universitaires de France, Paris, 1970,
  english translation available.

\bibitem{shende-strata}
V.~Shende, \emph{Hilbert schemes of points on a locally planar curve and the
  {S}everi strata of its versal deformation}, Compos. Math. \textbf{148}
  (2012), no.~2, 531--547.

\bibitem{vainsencher-10}
I.~Vainsencher, \emph{Enumeration of {$n$}-fold tangent hyperplanes to a
  surface}, J. Algebraic Geom. \textbf{4} (1995), no.~3, 503--526.

\bibitem{verdier-whitney}
J.-L. Verdier, \emph{Stratifications de {W}hitney et th\'eor\`eme de
  {B}ertini-{S}ard}, Invent. Math. \textbf{36} (1976), 295--312.

\bibitem{claire-miroir}
C.~{Voisin}, \emph{{Sym\'etrie miroir}}, Paris: Soci\'et\'e Math\'ematique de
  France, 1996.

\bibitem{YZ}
S.-T. Yau {\normalfont \smfandname} E.~Zaslow, \emph{B{PS} states, string
  duality, and nodal curves on {$K3$}}, Nuclear Phys. B \textbf{471} (1996),
  no.~3, 503--512.

\bibitem{yifan_zhao}
Y.~Zhao,
\emph{Stable maps and Euler characteristics of compactified Jacobians},
to appear.

\end{thebibliography}


\end{references}

\stopcontents[panoramico]



%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main.tex"
%%% coding: utf-8
%%% End: 
 	

